Large Language Models for User Interest Journeys

Large language models (LLMs) have shown impressive capabilities in natural language understanding and generation. Their potential for deeper user understanding and improved personalized user experience on recommendation platforms is, however, largely untapped. This paper aims to address this gap. Recommender systems today capture users' interests through encoding their historical activities on the platforms. The generated user representations are hard to examine or interpret. On the other hand, if we were to ask people about interests they pursue in their life, they might talk about their hobbies, like I just started learning the ukulele, or their relaxation routines, e.g., I like to watch Saturday Night Live, or I want to plant a vertical garden. We argue, and demonstrate through extensive experiments, that LLMs as foundation models can reason through user activities, and describe their interests in nuanced and interesting ways, similar to how a human would. We define interest journeys as the persistent and overarching user interests, in other words, the non-transient ones. These are the interests that we believe will benefit most from the nuanced and personalized descriptions. We introduce a framework in which we first perform personalized extraction of interest journeys, and then summarize the extracted journeys via LLMs, using techniques like few-shot prompting, prompt-tuning and fine-tuning. Together, our results in prompting LLMs to name extracted user journeys in a large-scale industrial platform demonstrate great potential of these models in providing deeper, more interpretable, and controllable user understanding. We believe LLM powered user understanding can be a stepping stone to entirely new user experiences on recommendation platforms that are journey-aware, assistive, and enabling frictionless conversation down the line.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> Paper_ Extracting and Naming User Journeys for Companion Recommenders (3)/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> Paper_ Extracting and Naming User Journeys for Companion Recommenders (3)/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> Paper_ Extracting and Naming User Journeys for Companion Recommenders (3)/abstract.tex <==
Large language models (LLMs) have shown impressive capabilities in natural language understanding and generation. Their potential for deeper user understanding and improved personalized user experience on recommendation platforms is, however, largely untapped. This paper aims to address this gap.
%\minminc{talk about the current problems in recsys we are trying to address.} 
Recommender systems today capture users' interests through encoding their historical activities on the platforms% (using sequence models)
. The generated user representations are hard to examine or interpret. On the other hand,  if we were to ask people about interests they pursue in their life, they might talk about their hobbies, like \emph{I just started learning the ukulele}, or their relaxation routines, e.g., \emph{I like to watch Saturday Night Live}, or \emph{I want to plant a vertical garden}. %In contrast, current recommendation systems don't have this reasoning \minminc{the word "reasoning" could trigger asks about reasoning related literature} capability. 
We argue, and demonstrate through extensive experiments, that LLMs as foundation models can reason through user activities, and describe their interests in nuanced and interesting ways, %the interest journeys users are pursuing, 
similar to how a human would. %This in return can enable entirely different user experience on recommendation platforms. \minminc{might want to discuss this in conclusion section.}

%alalama re-wrote: {Among all the user interests, we define the persistent and overarching, in other words the non-transient ones, as journeys. These are the ones we believe will benefit most from such nuanced and personalized descriptions and the downstream new user experiences enabled. }
We define \emph{interest journeys} as the persistent and overarching user interests, in other words, the non-transient ones. These are the interests that we believe will benefit most from the nuanced and personalized descriptions. %, which will in turn enable downstream new user experiences.
%\minminc{konchris to validate the above journey definition.} 
We introduce a framework in which we first perform \emph{personalized} extraction of interest journeys, and then summarize the extracted journeys via LLMs, using techniques like few-shot prompting, prompt-tuning and fine-tuning.  %We find that prompt tuning LLMs on a small dataset of only 60 examples from a proxy domain of expertly curated and named collections can do a great job in naming user interests. 
Together, our results in prompting LLMs to name extracted user journeys in a large-scale industrial platform demonstrate great potential of these models in providing deeper, more interpretable, and controllable user understanding. We believe LLM powered user understanding can be a stepping stone to entirely new user experiences on recommendation platforms that are \emph{journey-aware}, assistive, and enabling frictionless conversation down the line. %and can enable truly conversational recommender systems based on deeper user understanding. % and can assist users throughout their life journey. This should also have significant applications to enable truly conversational recommender systems that can reason through user interests.


%We argue that for recommender systems to better assist users on their  journeys, they first need to be aware of them. In this paper, we focus on how to extract the journeys a user is pursuing. We use a large-scale industrial recommendation platform as our case study. We first conduct a user study to understand whether and how users use the platform to pursue their long-term journeys. We formalize the problem, propose a journey extraction service, and present a personalised clustering algorithm instantiating the service. By defining the desired properties for the extracted journeys, we evaluate different approaches that can be used for the clustering algorithm and share insights. We demonstrate qualitatively and quantitatively that the extracted user journeys are of high quality, opening the door for journey-aware recommendations.

%People use recommendation systems to get help on making a variety of choices in their everyday life. While the classic recommendation paradigm of getting help on where to eat, what to shop, or which movie to watch is abundant, recently the range of choices users make with the help of recommendation systems has largely expanded. For example, users might be using the same platform to get content related to learning languages, playing instruments, setting up their own business, and so on. These are all interests that might be manifesting over the period of multiple interactions, over multiple days, months, or even years. 

%We argue that for recommendation systems to assist users towards these long-term interests that users enjoy spending time on, we need to make them aware of the journeys users are pursuing towards them. In this paper, we turn our focus into    how to extract these user journeys in the first place. We use a large-scale industrial recommendation platform as our case study. We perform user interaction research to understand to what extent and for how long users pursue long-term interests in the platform. Informed from the findings that more than half of users utilise the platform to pursue their long-term interests for more than a month, we formalise user journeys, and argue for the need of a journey extraction service. After specifying desired properties for extracted journeys, we translate the problem into a personalised clustering one. We show qualitative and quantitative results showing that the journeys extracted are high quality, which opens the way to future work of journey-aware recommenders.  

==> Paper_ Extracting and Naming User Journeys for Companion Recommenders (3)/conclusions.tex <==
Our work aims to bridge the gap in LLMs for understanding user interest journeys and improving user experience on recommendation platforms. We provide the first-ever demonstration of LLMs to reason through user interests and describe them similarly to how people would. We uncover important aspects to enable such capabilities, such as data, prompting techniques, and evaluation methodology. %which data to use to align LLMs with the interest domain, which prompting techniques work best, and how to evaluate generated names in the case of unlabeled user histories. 
We show that prompt-tuning LLMs based on small but quality data of expertly curated and named collections has the most generalization capability. We also find first extracting the interest journeys through a personalized clustering procedure is critical. %We show that our proposed clustering method can uncover the longest most-coherent journeys, as opposed to non-personalized baselines typically used in production systems.% Lastly, we provide some early results indicating the headroom of making recommendations aware of the uncovered human-interpretable user interest journeys, which paves the way towards journey-aware recommenders that provide more user control. 
We validate our findings on a large-scale industrial recommender platform, and together suggest the promise of utilizing our proposed journey service as a way to gain deeper user understanding and building novel user experiences that offer more user control. 
%In this paper, we have developed a method to extract personalized user journeys. Given a user and their interaction history with a recommender platform, our method decomposes the history into journey clusters; each containing the sub-sequence of interactions all around the same highly-valued interest. Our method by extracting journeys in the infinite concept space, can uncover deep semantic relations among items, and can be accessibly interpreted by users, as each journey is associated with top concepts describing it. Our evaluation of extracted user journeys from user interactions with  a large-scale recommender platform reveals the superiority of our method compared to state-of-the-art non-personalized clustering approaches. Our method can extract significantly longer, denser journeys, at the right granularity, while providing interpretability and alowing intra-journey comparison, and item-journey comparison; unlocking future research for journey-aware recommendation. 

%Our next step is to evaluate the usefulness of our extracted journeys to the recommendation process. This opens the door to journey-aware recommenders that can accompany the users throughout their lifelong interactions with the platform. To further enable these companion recommenders, in future work we plan to name the journeys through open-form natural language, rather than set of concepts. We also hope to develop journey-aware recommenders that can deliver recommendations tailored to their evolving journeys, and identify novel branches of interest journeys for users to consider exploring. 

%In future work, we want to further improve interpretability by naming journeys through open natural language,   

%We find that our method can find longer, denser journeys, accurately retrieving items from the user interaction history into the same journey cluster, while also providing good interpretability and allowing easy intra-journey comparison and item-journey comparison. They significantly outperform methods that are long-used in industrial recommender systems as ways to group content into unpersonalized categories.  

%Avenues of future work include:
%\begin{itemize}
%    \item naming of journeys.
%    \item Live experiments to show that extracted journeys can indeed improve recommendation quality, and user experience via better control and organization by journeys.
%    \item While all these are valid journeys, we believe that companion recommenders must also have an understanding of the users' context within each interest in order to predict journeys at the right granularity users want assistance with. This area will be the focus of future work.
%\end{itemize}

==> Paper_ Extracting and Naming User Journeys for Companion Recommenders (3)/formulation.tex <==
%https://docs.google.com/document/d/1lXsP3k5EBeb1EmcXqtRw-mgpQRaadDH5vFFg9M1Rp4E/edit?resourcekey=0-fH4vTKfOoEq4N2xHwirkSw#
%We compare journeys with related work on  understanding and modeling {user needs}, {intent}, and {tasks}.

%\subsection{Definitions}

%\begin{definition}[User Journey]%\footnote{For the purpose of this paper, we will focus on extracting user journeys, and will defer to future papers extracting the stops of a user journey. }
%\fbox{\begin{minipage}{0.45\textwidth}
%\emph{A user journey is a sequence of user-item interactions spanning different periods of time, coherent around a certain user goal or need. Users can have multiple journeys at any time point and the journeys can be interleaving.}
%\end{minipage}}
%\label{def:1}
%\end{definition}

%\begin{definition}[Life-long User Journey]
%The lifelong journey of a user is the union of their journeys, which are (potentially) interleaving.
%\end{definition}

%\begin{definition}[User Journey Stop]
%A user journey can be recursively split into sub-journeys, or else journey stops\footnote{For the purpose of this paper, we will focus on extracting user journeys, and will defer to future papers extracting the stops of a user journey. }
%, capturing in a more granular level the sub-themes of a journey.
%\end{definition}

%\subsection{Discussion}
%\textbf{User Intent, Tasks, \& Needs.} 
\textbf{Intent, Tasks, User Needs} %\kc{Consider having them as not subsections}
We compare journeys with related work on  understanding and modeling {user needs}, {intent}, and {tasks}. Intents has long been considered in the search domain \cite{zhang2011user, radlinski2010inferring}. 
Recent works on intent-aware recommendation  \cite{bhattacharya2017intent, mehrotra2019jointly} shows modeling intent improves user satisfaction. 
While intent captures the high-level context of the user’s visit, it is much coarser than journeys. For example, the intent of "I want to do something inspiring" covers “becoming an entrepreneur” and “learning the ukulele” journeys. % Thus, we leave intent outside the scope of this paper, noting that knowledge of intent can help cut down the space of user journeys. 
Another related work is modeling task behavior, which goes beyond the current single query, in search engines to improve search ranking (e.g., \cite{white2013enhancing, lucchese2011identifying}). However, search tasks are typically based on in-session interactions \cite{lucchese2011identifying} or across  only a few sessions \cite{kotov2011modeling}, while users are found to pursue interest journeys for a month, or more. In addition, interest journeys also cover persisting interest such as entertainment, which is less task-oriented. %This makes the well-studied \textbf{session-based recommendation} paradigm not a good fit either for our problem setting \cite{li2017neural}. 
% \subsection*{User Needs} 
User needs in Web search were categorized in \citep{rose2004understanding, broder2002taxonomy, yin2010building} as transactional, navigational, or informational. A similar categorization on \emph{why} users utilize recommendation systems has not been defined. Our findings suggest a new dimension of user needs: the dimension of using recommenders alongside real-life interests and aspirations, i.e., learning new skills, entertainment, and sense of belonging. This confirms our insight that the recommendation process should be transformed to satisfy this additional need. Broadly speaking, the goals of journey-aware recommendation align with those of personal assistants \cite{guha2015user, sun2016contextual, song2016query, safavi2020toward} and context-aware recommenders \cite{baltrunas2011matrix}. Our journey extraction technology can be utilized as context within a proactive personal assistant to tailor recommendations.

\textbf{User Interests Modeling}  Another close line of work is user modeling in recommender systems, and particularly modeling changing user interests via sequential models (e.g., RNNs) on user actions \cite{wu2017recurrent, chen2019top}. %However, there are a few key differences between user journey and user interest: 1) user journeys span across multiple user interactions while there can be fleeting user interests with one-off interactions; 2) user journeys are across contents that are valued by the user, i.e., those addressing their real life needs and goals, and excluding regretted interactions;  3) user journeys are highly personalized and capture the progression and evolution toward their needs or goals through interacting with contents. 
%\minminc{commented out the diff between interests and journeys.}
Although powerful, sequence models such as RNNs tend to focus only on the last interactions, forgetting long-term user interests. % In such cases, unless the user has recently interacted with content related to their journey, the model won't be able to tailor recommendations on the user's journey progress.
%\textbf{Attending to Long-Term history} 
%In addition, our approach offers additional interpretability, while the user representations provided by sequence models such as RNNs are hard to examine and interpret. 
To mitigate the recency bias, a recent thread has focused on incorporating users’ long-term history data into recommendation models \cite{pancha2022pinnerformer, pi2019practice, zhou2019deep} by powering models with attention-based mechanisms \cite{kang2018self, sun2019bert4rec}. The produced user representation however is hard to examine or interpret. In this work, we take a different approach: extracting longer-term valued journeys, separately from the recommendation task. This allows for modularity of involved components and for interpretability  \cite{radlinski2022natural}, to enable the system explain recommendations via the lens of journeys \cite{tintarev2007explanations}.
 Our journey extraction service allows to easily inspect and  control the granularity of extracted journeys, while naming each journey via LLMs makes our approach interpretable.  Furthermore, by introducing the journey entity, we can eventually enable users to interact with their extracted journeys; e.g., control whether they want more or less recommendations related to that journey. 
%\textbf{Topic Models \& Personalized Clustering}
Also, our approach of extracting journeys via clustering, while paying attention to content understanding is related to user topic modeling \cite{zaheer2017latent, bahrainian2019predicting, 37745} and clustering content by user needs \cite{kong2016improving, 49265}. Also, works on uncovering coherent trails \cite{chi2001using, shahaf2010connecting, shahaf2012trains, 49265} inspired us greatly.

\textbf{Interpretable/Transparent User Models} Our work is related to many past works advocating for the need of \emph{explainable recommendation} \cite{tintarev2007explanations}, as well as \emph{user control} \cite{jannach2017user}. Our contribution is the first-ever study showing the power of prompted LLMs so that they can reason through user interests; as well as shedding light to the angle of persistent real-life user journeys that users expect recommenders to help them with besides the shorter-term tasks. Perhaps the most close work to ours is 
%Furthermore, although there have been many past works advocating for the need of \emph{explainable recommendation} \cite{}, as well as interpretability in recommender systems \cite{}, the majority of the efforts have focused on explaining to the user the inner workings of the recommender \cite{}. Rather, our focus is on exposing to users a human-readable and interpretable summary of their persistent interests, with ultimate goal to provide them more control, which has been shown to lead to higher satisfaction \cite{}. We will further validate that by follow-up work where we plan to provide these uncovered and named journeys in user facing live experiments, and map them to recommendations, allowing the users to to be assisted with their journeys when they want.
\cite{radlinski2022natural} which laid out the vision for
scrutable Natural Language (NL)-based recommendation. 
%Our approach of naming the users' interest journeys in order to make recommendations journey-aware is the most similar in principle to the vision laid out in  . Both works advocate for the need of the usage of natural language to provide succinct summaries of user interests, similarly to how humans would describe them. 
Our work however has several differences: Rather than a complete summary of user interests, we aim at short sentences describing different user interest journeys. Also, while \cite{radlinski2022natural} focuses on scrutable profiles, with the aim of recommendation, we focus on investigating the degree to which our personalized clustering approach coupled with prompting LLMs can provide deeper user understanding. Perhaps the most important difference is that, to our knowledge, our work is the first-ever experimental study of aligning LLMs to reason through user journeys. Furthermore, our work differs significantly from \cite{balog2019transparent} where the authors showed how a restricted representation of users as weighted pairs of tag interaction can be verbalized as NL statements using templates. Our models rely on free-form natural language, rather than templates to output interest names.% such as "hydroponic gardening", "ukulele for beginners", "advanced woodworking techniques".

\textbf{Large Language Models (LLMs)} Last but not least, our work is the first to demonstrate the application of LLMs in the user interest journey domain, for deeper user understanding in recommendation systems. While \cite{radlinski2022natural} provided some key directions along the usage of LLMs in the recommendation space as mentioned above, to our knowledge this is the first study to address issues like which data to use to fine-tune and prompt-tune LLMs to align them with this domain, how different prompting techniques perform, among others. We argue that there is large untapped potential in LLMs for the domain of recommender systems. We know that recent large pre-trained language models have been shown to have impressive generative fluency \cite{thoppilan2022lamda, chowdhery2022palm} as well as effective few-shot learning capabilities \cite{brown2020language} in the domain of natural language generation and understanding, and have passed several benchmarks of various tasks. However, so far, the key application to the recommendation system domain has been the P5 paper \cite{geng2022recommendation} which effectively maps recommendation as a language processing task, framing a variety of recommendation tasks into an end-to-end transformers framework. %However, that work has a significantly different take-away, i.e., framing a variety of recommendation tasks, such as sequential recommendation, rating prediction, review summarization, explanation generation, into an end-to-end transformers framework \cite{} using a multitask collection of personalized prompts. 
Our work is orthogonal; it leverages the power of LLMs as a way to reason through user interests, so to provide the interpretability a human would offer if they were to be asked for a recommendation. 

%There has been a lot of recent interest in modeling user intent into recommendation systems \cite{}; where intent captures at a high level what the user might have in mind/need from their current visit. The key distinction between intent and user journey is on granularity; with intent being a more coarse way to cut down the space of recommendations, and journeys being more granular. For example, an intent of "I want to learn", or "I want to do something inspiring" doesn't distinguish between a <study how to be an enterpreneur> or the <learn to play the ukulele> journey. While intent is  crucial in companion recommender systems, given it's significantly different from journey extraction, we leave it outside the scope of this paper.\footnote{ Predicting user intent could further help cut down the space of user journey.} 



%Another recent line of work has focused on including the long-term history of a user into the recommendation models, and improving the underlying models to better leverage this history. There are two main differences between this and user journeys extraction. One, the latter should be more interpretable; we can control the granularity, and we can easily inspect user journeys, and content metadata about such journeys. Two, by introducing the journey entity, we can allow the user to eventually interact with it, and have user feedback on journey propagated to all items related to this journey. 

%\textbf{User Journey vs User Interest:} %For a user interest to become a user journey, there need to be: (1) multiple user interactions and (2) some notion of users' satisfaction of interacting with this interest. A user journey can then be framed as a sequence of interactions of the user with items all about a highly valued interest, or else interactions with a \emph{sticky high-valued interest}. This excludes one-off interactions, or interactions a user didn't value afterwards. Furthermore, user interests as typically considered by state-of-the-art recommenders at the level of e.g., "ukulele", where every item related to ukulele recommended to the user would be a good fit. In contrast, a user journey is supposed to capture the highly personalized evolution of a journey, capturing the variability of interest progression from person-to-person based on e.g., their acquired skill and progress. In a nutshell, \emph{User journey is a fine-grained interest that evolves in a personalized way and can be associated with one or more intents.}


%as a multi-session interaction sequence of a highly valued interest (or sticky high-valued interest). 

%Furthermore, we wish to capture the granularity and context of interest descriptions. For example, currently, a recommender might describe a person’s interest as "ukulele," – but in real-life scenarios, this interest might be highly variable from person-to-person, based on their acquired skill and progress.


%For a user interest to justify as a journey towards this interest, there need to be: (1) multiple user interactions, (2) some notion of satisfaction of the users by interacting with items from this interest. Thus, another way to frame user journey is a sequence of user-item interactions all about a highly valued interest, over multiple interactions, or else interactions about a \emph{sticky high-valued interest}. This excludes one-off interactions, or interactions a user didn't value afterwards. Another key distinction is that interests in recommender systems are typically defined in the level of "ukulele" in which case every content item recommended to the user related to ukulele would be considered a good fit. However, what "ukulele" interest means to one user is quite different from what it means to another. For instance, users' acquired skill, and progress while interacting with ukulele content, will make two ukulele journeys of two users potentially very different. 


==> Paper_ Extracting and Naming User Journeys for Companion Recommenders (3)/introduction.tex <==
%While the classic recommendation setup involves helping users decide \emph{at the moment} where to eat, what to buy, or which movie to watch, the role of recommendation systems has widely expanded to support a variety of real-life goals and tasks. Users might rely on the same platform to find content related to planning a trip, learning languages, playing instruments, setting up their own business, and so on. User journeys can span a much longer time horizon over multiple days, months, or even years, and involve many interactions with the recommender. Meanwhile, users can also be interested in pursuing a variety of different journeys. 


%People typically make choices in the context of their life needs and goals. 

With the abundance of the internet content, the role of recommendation systems has significantly expanded. % across different areas of one's life. %we've seen a paradigm shift. 
In the past, users mainly relied on recommendation systems to make %faster, easier 
one-off decisions around where to eat, what to buy, or which movie to watch \cite{koren2009matrix, sarwar2001item, covington2016deep}. Nowadays, users expect the recommendation platforms to also support their persistent and overarching interests, including their real-life goals that last days, months or even years \cite{liang2023enabling, liang2019recommender, ekstrand2016behaviorism}. %from the platform to not only support their interests, i.e., knowing their underlying preferences to help them decide what to watch/read tonight, but they also support tasks for the shorter term %(like getting occasional decoration tips, or making their vegetable garden thrive)
% as well as longer-term goals. % (from learning the ukulele, to starting a business).
For example, a user who is into stand-up comedy would want recommendations tailored to their  tastes, and might expect the system to help them explore other forms of comedy performance. A user who is learning to play an instrument or is improving home decoration, would want recommendations and tips appropriate to their skill level. Or, a user with the goal of becoming an entrepreneur would want the recommender system to find inspirational content assisting them every step along the way. % Similarly, when a certain task arises, such as improving home decoration, or how to grow vegetables, they might need helpful tips.

If one were to ask a friend for recommendations around any of their journeys, %advice around any of these shorter to longer-term tasks, 
the friend would probably ask them to first describe their interests or needs in detail. %a clarifying question to get a nuanced description of the actual user need, or task or goal they want to accomplish. 
%For a person to assist another with their needs and goals, the first step is typically to ask what they want to do, with the user then describing in a nuanced way what it is that they want to pursue. 
Once they get a reply, like \emph{I want to know the history of stand-up comedy and the most famous stand-up comedian at this time}, or \emph{I started playing ukulele a month ago, and I want to improve my strumming skills}, % \emph{making their vegetable garden thrive} or \emph{starting a business} or \emph{find something funny to relax}, 
the friend would then be in a much better position to give good recommendations. Conversely, recommender systems make recommendations by predicting the next item a user might want to interact with,  given their historical activities \cite{sarwar2001item, covington2016deep, beutel2018latent}. % given large amount of user-item interactions, what the next item a user might want to interact with now. But, what if what user wants is a function of their real-life journey, and their changing goals and tasks at hand?
%With this context, we argue for transforming the recommendation process to \emph{companion recommenders} enabled by extracting users’ long-term journeys.   % give advice is on the basis on current user needs, predicting what the next items  

We argue that this type of collaborative filtering based approach \cite{he2017neural, covington2016deep} does not meet user needs for higher-level semantic preferences. In order for recommender systems to truly assist users through their real-life journeys, %we need to first arm them with \emph{reasoning} capabilities around 
they need to be able to understand and reason about interests, needs, and goals users want to pursue \cite{radlinski2022natural, guha2015user, mehrotra2019jointly, sun2016contextual}. However, the task presents some challenges. First, users often do not explicitly spell out their interests, needs, and real-life goals to the recommenders. As a result, the recommenders need to infer them from the historical activities the users engaged on the platform. Second, users can have multiple journeys intertwined in their activity history at any time. Third and most importantly, journeys are personalized and nuanced. Two users who are both into stand-up comedy can be interested in completely different aspects of it (e.g.,  \emph{history of stand-up comedy documentaries} vs \emph{Saturday Night Live skits}). %Third, these goals and tasks change and complete as their journeys evolve, which needs to be automatically detected by the system \kc{change}.
This is where Large Language Models (LLMs) come in play. LLMs have demonstrated impressive capabilities for natural language understanding and generation, achieving state-of-the-art performance in a variety of tasks, from coding to essay writing to question answering \cite{brown2020language, thoppilan2022lamda, chowdhery2022palm, chung2022scaling}. What if we power recommender systems with LLMs that can reason through user activities on the platform to uncover the underlying personalized and nuanced user interests, needs and goals, that is: user journeys?  %that can reason through user actions, and uncover the underlying user needs, tasks and goals? 
%Making companion recommenders a reality however faces significant challenges. First, users often do not explicitly name their real-life aspirations to the recommenders. Second, users can have multiple goals and tasks intertwined at any time. Third, these goals and tasks change and complete as their journeys evolve, which needs to be automatically detected by the system. \kc{Make this more aligned with our solution.} %and the users don’t explicitly say when they are done with them. 

To this end, we propose to build a personalized user journey profile which 1) uses personalized clustering to uncover coherent \emph{user journeys}, i.e., persisting user interests, needs, and goals, from a long sequence of user interaction logs, and 2) leverages the capabilities of LLMs aligned to the user interest journey domain through prompt-tuning \cite{lester2021power} and fine-tuning \cite{ziegler2020finetuning} on different data sources, to describe the extracted journeys with interpretable and nuanced names. Together, we make the following contributions:
%based on large-scale interaction logs, and name extracted journeys via prompting LLMs.
%Particularly, 
%given the large-scale noisy interactions users have with different items, we first extract in a personalized fashion groupings of the underlying user needs, which correspond to what we refer to as \emph{user journeys}. Then, for the LLMs to be aligned to the domain of user interest journeys, we propose different types of data based on which we can do prompt tuning and fine-tuning to allow the models to give good interest names. We then utilize the journey-aligned LLMs to infer the user interest name on top of the extracted journey cluster.  Together, our contributions are: \kc{refine and make shorter.}
\begin{itemize}
    \item A first demonstration of the capabilities of LLMs to uncover and describe in natural language the interests, needs, and goals users pursue, similar to how people would describe them, e.g., \emph{hydroponic gardening}, \emph{playing the ukulele as a beginner}, \emph{cooking italian recipes} (Figure \ref{fig:journey_service}). We posit that this will unlock unique user experiences and enable recommenders to assist users throughout their journeys.
    \item A thorough research study shedding light into the different factors impacting the quality of the generated journey names, e.g., the prompting techniques, the underlying domain data used for prompting, the LLM architecture and size, and the journey extraction technique. % This should shed light into the capabilities of foundational models in providing nuanced human-like interest journey names. 
    \item An at-scale user research study uncovering the taxonomy of real users' journeys and how they pursue them on recommendation platforms.  
\end{itemize}
%longer-term interests like 
%can use recommender platforms from finding the content they want right now, to finding 
%pursue different real-life goals, from, to getting .
%to support a variety of real-life goals and tasks
%The abundance of  internet content and the prevalence of personalized recommenders have led to a paradigm shift. The same user can use the one platform for multiple real-life goals simultaneously – including 
%Thus, a key research direction is in designing recommenders that can assist users in these user journeys on top of one-off interactions. 
%Specifically, what these user journeys are, how can we extract them from the noisy implicit user interactions and how can we name them in a similar fashion as users would describe them.  To answer these questions, we offer a number of contributions: First, a large-scale user study on whether indeed users use recommenders to pursue their long-term journeys, and how they pursue them. Second, a formalization of journey extraction as a personalized clustering problem. Third, a novel way to label user journeys in an interesting way via prompting large language models, based on both prompt engineering and tuning the prompt embeddings on small high quality data. Fourth, using as our case study a large-scale industrial recommender platform, an evaluation of journey extraction and journey naming. Together, these contributions pave the way to recommenders that are aware of users long-standing journeys, and can assist them throughout their lifelong journey on the platform.
%\kc{alalama: do we need Fig 2? can we list some Fig 2 journeys and taxonomy so it takes less space? }
\begin{figure*}[!t]
    \centering
    \includegraphics[scale=0.35]{images/journey_service.png}
    \caption{Our approach uses personalized clustering to uncover coherent user journeys, and names them via prompting LLMs.}
    \label{fig:journey_service}
\end{figure*}
%People typically make choices in the context of their life needs and goals. For example, when someone learns to play an instrument, they want to get advice from their instructor adapted to their skill level and knowledge so far. Or, when one has the goal of becoming an entrepreneur, they want to find content that inspires them, guiding them each step of the way to reach their goal. Similarly, when a certain task arises, such as improving home decoration, or how to grow vegetables, they might need advice on how to accomplish this task. 
%The abundance of content on the internet, together with creators producing content and making it available in content recommendation platforms, has led to a paradigm shift into how recommendation systems are used. The same user can use the same recommendation platform for all the scenarios above. They have a real-life goal of learning the ukulele, and they want to start their own business; but they also need once in a while decoration tips and when their garden is not looking optimal learn advice on how to make their vegetables thrive. 
%So far, the application of LLMs on the recommendation domain is largely focused on reframing existing tasks like rating prediction, or sequential item prediction in the Transformers transfer learning setting. However, there has been little to no precedent in exploring  LLMs' capabilities in a more thorough user understanding, and increased interpretability. 
%Existing recommender systems curate contents based on what the user wants at the current moment. %But what if the user wants to evolve or modify their goals and tasks at hand? 
%But what if what the user wants is a function of their real-life journey, and their changing goals and tasks at hand?
%With this context, we argue for transforming the recommendation process to \emph{companion recommenders} enabled by extracting users’ long-term journeys. 
 %. This way, they can truly accompany the users over their real-life evolving goals and tasks.  
%This leads to a paradigm shift of recommender systems. The promise of the recommendation process is to help curate content based on what the user wants at the current moment. But what if what the user wants is a function of their real-life journey, and their changing goals and tasks at hand? With this context, we argue for a transformation of the recommendation process to \emph{companion recommenders}. To enable this vision of companion recommenders, a crucial component is to extract the users’ long-term journeys. We argue that by knowing the bigger journeys users are on, and which ones they might want help with, we can adapt recommendations so that they are no longer a function of only current user needs, but also bigger journeys towards goals / tasks users are pursuing. 
%Thus, a key research direction is in designing recommenders that can assist users in these user journeys on top of one-off interactions. Specifically, what these user journeys are, how can we extract them from the noisy implicit user interactions and how can we name them in a similar fashion as users would describe them.  To answer these questions, we offer a number of contributions: First, a large-scale user study on whether indeed users use recommenders to pursue their long-term journeys, and how they pursue them. Second, a formalization of journey extraction as a personalized clustering problem. Third, a novel way to label user journeys in an interesting way via prompting large language models, based on both prompt engineering and tuning the prompt embeddings on small high quality data. Fourth, using as our case study a large-scale industrial recommender platform, an evaluation of journey extraction and journey naming. Together, these contributions pave the way to recommenders that are aware of users long-standing journeys, and can assist them throughout their lifelong journey on the platform.


%\begin{itemize}
%\item \textbf{Journey Extraction via co-embedding of journeys and items, and personalized clustering:} By embedding both journeys and items into the same infinite embedding space, we propose a personalized clustering approach using distance on the embedding space as a way to disentangle journeys. %and items associated with the overarching journeys. 
%\item \textbf{Journey Naming via prompt-engineering and prompt-tuning LLMs:} We tackle the issue of sparsity of journey labels via crowdsourcing based on user interviews and proxy domain data. We show that prompt tuning LLMs like LaMDa and PaLM based on small quality data can provide human-like names for user journeys.
%\item \textbf{Case Study in Large-Scale Industrial Platform:} We show that our techniques can successfully retrieve long coherent journeys, with much better recall compared to non-personalized journey extraction methods. We also find that prompt-tuning LaMDa 137B model based on small data of collections curated and named by experts has good generalization capability in naming real user journeys. 
%both quantitatively and qualitatively the extracted and labeled journeys, and show that our approach can effectively transform noisy interaction histories into journeys of the right granularity, with human-like names.
%\item \textbf{At-Scale User Research on user journeys:} We provide the first taxonomy of real users' valued journeys and how users pursue them in recommendation systems, %, providing another finer dimension to categorize user needs than the seminal categorization of navigational,  informational, or transactional.
%\end{itemize}

%Overall, this proposed framework of the journey extraction and naming service shown in Figure \ref{fig:journey_service} allows for a deeper user understanding transforming the noisy interactions to small sentences describing the underlying user needs/task/goals (e.g., \emph{hydroponic gardening}, \emph{playling the ukulele as a beginner}, \emph{cooking italian recipes}), similarly to how people would describe them. We posit that this work enables journey-aware recommenders, that can map what the system recommends to the user's underlying interests, tasks, and goals. It also demonstrates the reasoning capability of LLMs for the domain of personalisation, that can unlock unique user experiences.
%\kc{potentially remove}By introducing this new entity of journeys to the classic setup of users-items (and their associated metadata) we pave the way forward to journey-aware recommenders: recommenders can help users find contents tailored to their journey, allow users to control whether they want to see more or less of contents related to a journey and to explore related journeys 

%This introduces a new entity to the classic recommendation paradigm besides users, items, and their associated features: the entity of \emph{journeys}. With this new capability to capture user history and to organize contents by journeys, recommenders can help users find contents tailored to their journey, allow users to control whether they want to see more or less of contents related to a journey and to explore related journeys. We make the following contributions:
%\begin{itemize}
%    \item \textbf{User Research study at-scale on whether, how, and for how long users pursue interest journeys} in an industrial recommender platform (Section \ref{sec:uxr}). To the best of our knowledge, this is the first-ever such study, revealing a taxonomy of valued journeys, and providing another finer dimension to categorize user needs than the seminal categorization of navigational,  informational, or transactional.
%    \item \textbf{Problem formulation} of journey-aware or \emph{companion} recommenders, along with key definitions and components needed (Sections \ref{sec:formulation}, \ref{sec:journey_service}).
%    \item \textbf{Novel method for personalized journey extraction}, which uncovers journeys by representing them into an infinite concept space where both journeys and items live (Section \ref{sec:methods}).
%    \item \textbf{Qualitative and Quantitative evaluation} of user journeys extracted from interactions with a large-scale industrial platform, showing the promise of our approach compared with commonly adopted co-occurrence and topic-based clustering methods (Section \ref{sec:results}).
%\end{itemize}
%Together, these contributions unlock future research work to reach the vision of companion recommenders.

%We start with a more formal problem definition (Section \ref{sec:formulation}), introducing key concepts which will be useful to contrast journeys to related but different concepts of interests and intent. We perform user interviews at scale to understand whether, how, and for how long users indeed using recommendation systems along side their interest journeys (Section \ref{sec:uxr}). We describe in more detail the journey service we propose alongside its intended benefits (Section \ref{sec:journey_service}). We then focus on the key question of how to extract the journeys (Section \ref{sec:methods}), and provide both qualitative and quantitative results to showcase that our method is simple yet effective in uncovering bigger threads of content users are interested in (Section \ref{sec:results}). We compare the proposed approach to related work (Section \ref{sec:related_work}) and conclude the paper with remarks on future work journey user profiles unlock to come closer to the vision of companion recommender systems (Section \ref{sec:conclusions}). 

%Let’s take a user coming to a large-scale recommendation platform, and take a look at their lifelong journey on the platform, and how we can best assist that. Besides their interests at the moment, users might have some real-life goals to accomplish─maybe they want to learn to play the ukulele, and educate themselves about climate change and entrepreneurship, to eventually build their own environmental startup;
%Maybe they have a task in hand, e.g., comparing different camera products to make a purchase or acquiring information on how to bring a puppy home; Maybe there are times they simply want to relax or explore and discover new channels. Some of these sub-journeys span years or months, some across days, and others are completed within a session. Meanwhile, depending on what they’re doing in parallel, they might want very different types of content when progressing on these sub-journeys. For example, in the ukulele journey instance, when driving to work they might want to listen to songs from ukulele professionals for inspiration, versus at home when relaxing, they might want to watch ukulele tutorials for their skill level. 

%We aim at building a companion recommendation system that can assist the users in their lifelong journey. To this end, we need to determine which sub-journey the user is at at any moment in time and understand the context and environment the user is in, and find the content best matching their current progress of each sub-journey and their context. 

%https://docs.google.com/document/d/1iPEWGY7qEz8RRYEri3ZVw8Q49-RayPZpWBleVCkdMBc/edit?resourcekey=0-sViJfuD4WAdcv2UrUDkxaw#heading=h.yujt76fa44t5




==> Paper_ Extracting and Naming User Journeys for Companion Recommenders (3)/journey_service.tex <==
%\kc{TBD{cjadams for overview, and main components}}

% Together the user study insights suggest the importance for our methods to both extract and name user interests in the right granularity, and to have natural language capturing the right nuance of the journey users are indeed pursuing. This is already prescribing the solution we propose, and our design criteria, which we further delve into in what follows.
%The user study insights motivate us to build journey-aware recommendation experience which allows users to interpret and control recommendations to better pursue their interest journeys.

\subsection{Overview}
\label{sec:method:overview}

\textbf{Journeys.} 
%Before we proceed with the specifics, let us first define the term 
We first define \emph{journey} as the umbrella term for user interests, needs, and goals: \emph{a user journey is a sequence of user-item interactions spanning different periods of time, coherent around a certain user interest, need or goal}. Users can have multiple journeys at any time point, and the journeys can be interleaving.

\noindent \textbf{Journey-aware recommendation.} We envision a journey-aware recommender system,  capable of identifying personalized user interest journeys and making recommendations accordingly to assist these journeys. %that is accompanying the user throughout their lifelong journey. Such a system would be capable of identifying and supporting personalized, long-term user journeys, and then mapping them to the right items supporting this journey. 
% In this work, we focus on the user understanding piece of uncovering and naming the journeys users pursue, which we refer to as \textbf{journey service}. In follow-up work, we will focus on mapping these extracted and named interest journeys to recommendations. 


% \begin{wrapfigure}{l}{0.4\textwidth}
% \begin{minipage}{.39\textwidth}
%         \includegraphics[width=\textwidth]{images/video_game_strategy_viz.png}
%         \caption{Visualization of journeys across users, with each point representing an extracted and named journey. We generate embeddings for each journey name through Universal Sentence Encoder \cite{cer2018universal} and cluster them with UMAP \cite{mcinnes2020umap}. Highlighted, a \emph{video game strategy} journey and its nearest neighbors in the embedding space, per cosine similarity.%\minminc{the annotation here are using salient terms, is it better to use llm generated names?} %Visualization of journeys across users, with each bubble representing an extracted infinite concepts journey. We generate embeddings through Universal Sentence Encoder \cite{cer2018universal} for the top 5 terms of each journey with at least 5 items and cluster them with UMAP \cite{mcinnes2018umap}. Highlighted, a journey with terms [hacks, woodworking, wood, garden, gardening] and its nearest neighbors in the embedding space, per cosine similarity.
%         }
%         \label{fig:journey_visualization}
%     \end{minipage}%
% \end{wrapfigure}

Here we focus on the foundation work of extracting and naming user interest journeys, referred to as \textbf{journey service}, and leave mapping these extracted and named journeys to recommendations for future works. 
%\subsection{Journey Service Components}
The proposed journey service consists of two components, as illustrated in Figure \ref{fig:journey_service}: 
\begin{enumerate}
    \item \textbf{Journey Extraction:} Maps the sequence of noisy interactions a user had with items on the platform into coherent journey clusters. % These journey clusters describe user journeys %in a variety of topics, i.e., entertainment, education, or long-term personal hobbies as uncovered 
    % falling under the valued journeys taxonomy. They can be pursued over interactions spanning different time periods, with singleton journeys containing only a single user-item interaction being removed.
    The journey clusters span different time periods, with singleton journeys (i.e., containing only a single user-item interaction) removed.
    \item \textbf{Journey Naming:} Maps the extracted journey clusters to human-readable, nuanced journey names based on content metadata, such as \emph{hydroponic gardening}, \emph{playing the ukulele as a beginner}. This enables users to comprehend how the system understands their journeys, and gives them control over their recommendations (e.g. they can choose more or fewer recommendations from a certain journey).
\end{enumerate} 
We study the necessity of these two components in section~\ref{sec:results} and 
\ref{sec:results_naming}.
% We will also evaluate in Section \ref{add-here-reference} whether we need two components, or we can simply task the LLM with both extraction and naming of the user journeys.
%\subsection{Desired Journey Properties}
Our user research uncovered properties we need to take into consideration when designing the journey service:



\noindent \textbf{(I) Granularity of journey clustering}. As revealed in the user surveys, journeys are personalized, thus defining the right granularity of journey clusters for all users is challenging. Measuring granularity quantitatively is hard, thus we propose to measure it via precision and recall, relying on proxy data (i.e., human-curated playlists) to align our journey clustering to how a person would define them (Section~\ref{subsec:analysis}).  
%We instead rely on proxy data (i.e., human-curated playlists) and precision/recall metrics as detailed in section \ref{subsec:analysis} to align our journey clustering to how a person would define them. %The extracted journeys should neither be too generic, nor too specific. For example, a \emph{ukulele} journey might be too generic, whereas a \emph{learning A, B, C chords in ukulele} might be more specific than needed to capture the entire journey. Rather a \emph{learning the ukulele for beginner player} strikes the right balance. Although this can seem pretty obvious qualitatively, measuring this in a quantitative fashion is challenging, as it requires knowing the granularity we are looking for, which is not the case. We propose to measure granularity via precision and recall\footnote{When too coarse, many journeys will be unnecessarily merged, thus increasing recall while deteriorating precision; When too fine-grained, precision will be increased (at its limit each interaction is a separate journey), but recall will suffer.}. Precision measures the fraction of well retrieved journey items in the cluster out of all items in the cluster, and can be computed if we were to tell if there is an odd item in the cluster. Recall measures the fraction of well retrieved journey items in the cluster out of items in the ground-truth history, which requires someone labeling each item in the user history with a corresponding journey label. This of course is super challenging. Thus, we rely on proxy metrics and proxy data where we do have labels as we'll describe in section \ref{add-link}.

%\begin{figure}[!tbp]
  % \includegraphics[scale=0.3]{images/woodworking journey viz 0.png}
%  \includegraphics[width=0.4\textwidth]{images/woodworking journey viz 1.png}
%  \includegraphics[width=0.4\textwidth]{images/journeys_visualization.png}
  % NEAREST NEIGHBORS IMAGE (separate so it fits side by side)
  % \includegraphics[scale=0.5]{images/woodworking - nearest neigbors.png}
%  \caption{ \kc{here provide the corresponding figure with LLM-provided name.}
%  }
  % REFERENCES:
  % https://www.tensorflow.org/tensorboard/tensorboard_projector_plugin
  % Universal Sentence Encoder paper: https://arxiv.org/abs/1803.11175
  % UMAP paper: https://www.nature.com/articles/s41586-019-0969-x#citeas
%  \label{fig:journey_embedding_viz}
%\end{figure}




\noindent \textbf{(II) Nuance} \& \textbf{interestingness of journey names.} We would like to name the extracted journeys in a nuanced and interesting way, just as how the user would have described their own journey. For example, \emph{hydroponic gardening}, or \emph{growing indoor plants} as in Section \ref{sec:uxr}. We measure the quality of the generated journey names w.r.t. (proxy) ground-truth using Bleurt score \cite{sellam2020bleurt}, as well as imputed specificity, interestingness scores \cite{thoppilan2022lamda}, and other dimensions (Section~\ref{sec:results_naming}).  %We want the journey names to be as if a human would have described the interest they are pursuing. This requires the use of natural language to describe the journeys, rather than using embeddings that don't have any meaning to users. While keywords describing the journey could be useful to get a first read at what the journey is at, it doesn't satisfy how a human would describe it \ref{fig:journey_embedding_viz} -- typically a real person would use a small phrase/sentence. While the phrase when a person is first asked can be generic, such as \emph{gardening}, as described from our in-person interviews (Section \ref{sec:uxr}), when further asked can have more nuance like \emph{hydroponic gardening}, or \emph{growing indoor plants}. This is the type of journey names we are aiming at; i.e., the name should be specific enough and interesting to capture all the nuance of the journey the user is pursuing. We can again measure the journey nuance qualitatively; however, for a quantitative evaluation, a human-in-the-loop measurement is required. We report both in our experiments, and also utilize imputation models predicting specificity, interestingness, and other dimensions, given ratings from another domain \cite{}.

\noindent \textbf{(III) Safety of journey names.} As we envision showing users the generated names and allowing them to control and refine their recommendations down the line, it is important that the generated names are safe \cite{thoppilan2022lamda}. We rely on imputed safety score to measure safety of the generated names. We find the safety of the journey name largely depends on the safety of the included items within the journey cluster (Section~\ref{sec:results_naming}). %Given the journeys with their corresponding names will be an object the user can interact with to further control and refine their recommendations, it is important that they follow responsible AI principles. One aspect that is quite important to be considered for generative AI output, as demonstrated in the \ref{LaMDA} paper, is safety. Again, for our measurement here, we rely on small qualitative data, as well as imputation metrics to evaluate the degree to which the generated journey names are safe. We find that largely the extent to which a journey name is safe is a function of the safety of the included items. As future work, we plan to rely on models that automatically rank potential responses based on safety and other scores, to further improve safety metrics. 

%Other dimensions we want to include regarding the generated names are safety, specificity and interestingness. 
%In this paper we consider the case where we only have access to offline interaction histories, and we want at a certain snapshot to provide the journeys users have interacted with. However, other properties important when deploying this in a large-scale industrial recommender are freshness, and being able to satisfy both old recurring interests, and new ones. Also, the journey names should be as fresh as possible, periodically updated when the journey representation becomes too different. We leave this for future work. 


%In this paper we focus on first transforming the user noisy interaction to long-term journey clusters with their corresponding nuanced names, with the goal of deeper user understanding. However, ultimately, the extracted and named journeys are to be used to make recommender systems journey-aware, i.e., delivering recommendations tailored to the journeys the user is  pursuing. Since the design goals of the journey service will largely define the desired properties for the resulting extracted/ named journeys, for the sake of completeness, it's worth specifying them:  
%\begin{enumerate}
%    \item[(D1)] Enable better recommendation quality and user experience
%    \item[(D2)] Enable better organization of content by journeys
%\end{enumerate}
%\label{sec:desiderata}

%We will focus on the piece of mapping journeys to recommendations  
%\subsection{Desiderata for journey entity extraction}

%\kc{Rephrase!} Both journey extraction and journey naming components rely on deep content understanding. We study different content attributes such as  infinite concepts, co-occurrence, and audio/visual features, as potential candidates for content understanding (Section \ref{subsec:baseline}, \ref{subsec:infinite_concepts})

%Such a recommender would require many components.  This paper focuses on two components, providing foundations for the others.

%\begin{itemize}

%     \item \textbf {1) Understanding contents}: User journeys on recommendation platforms are largely captured by the contents they interacted with. Thus understanding user journeys requires understanding the contents.  We study different content attributes such as  infinite concepts, co-occurrence, and audio/visual features, as potential candidates for content understanding (Section \ref{subsec:baseline}, \ref{subsec:infinite_concepts}). 

%    \item \textbf {2) Extracting user journeys}: Once identified good content attributes, we need a service to cluster a user’s content consumption history. These clusters can describe long-term journeys in a variety of topics, i.e., entertainment (“90s hip hop”) or long-term personal hobbies (“healthy Mediterranean recipes”), or education (“Understanding how things work”) (Section \ref{subsec:personalized_clustering}).
    
%    Once content understanding has been developed, we require a service that can extract from a user's history discrete clusters of content that have been part of a particular interest journey.  Journey clusters are all content related to a long term interest, and could range from entertainment topics (e.g. “stand up crowd work”, “90s hip hop”), long term personal hobbies (“learning classical guitar”, “Healthy mediterranean recipes”), or education 
%    \item \textbf {3) Naming journeys in human readable format}:
     %Once extracted user journeys from a user's history, we need a human-readable semantic representation of each journey to allow user control as well as communicate to users the system’s understanding of their journeys.
    %\item \textbf {4) Surfacing journey-specific recommendations}:
    %Delivering recommendations tailored to the journeys the user is currently pursuing. %the content users have consumed as part of their journey. 
    %\item \textbf {5) Progressing and expanding journeys}: 
    %Updating the recommender's understanding of a user's journey  based on interactions with recommended contents over time; Identifying novel and related journeys for a user to  explore.
%\end{itemize}



%\input{metrics_methods}

% \begin{algorithm}
% \caption{Journey Extraction via Salient Terms for User $u$}\label{alg:cap}
% \label{algorithm:sts}
% \small{
% \begin{algorithmic}
% \Require ${\cal H}_u = \{i_t, t=1, \cdots, T\}$ containing list of items the user $u$ interacted with; salient terms similarity threshold $\epsilon: [0, 1]$; $M$: Minimum number of items per cluster. Default values: $T=0.1, M=1$.
% %\Ensure $y = x^n$
% %\State $y \gets 1$
% %\State $X \gets x$
% %\State $N \gets n$
% %\While{user $u$}

% %\State $\text{Journey}_1 = \{i_1\}$
% %\State first item $i_1$
% \State $\text{Journey}_1 = \{i_1\}$; Journey Set = $\{\text{Journey}_1\}$ 
% %\While{item $i \in$ Interaction History $H$ of user $u$}
% \For{item $i \in$ Interaction History $H$ of user $u$}
% \For{journey $j$ in Journey Set} 
% \State ItemJourneySim($i, j$) $\gets$ Cosine similarity between item $i$ and journey $j$
% \EndFor
% \State $j^\ast$ $\gets$ $\arg\max_{j'\in \text{Journey Set}}$ ItemJourneySim($j'$, $i$) 
% \If{ItemJourneySim($j^\ast$, $i$)>= T}
% \State {Add item $i$ to the journey, and update journey's salient term representation, based on salient terms of item $i$.} 
% \Else{}
% \State {Start a new journey composed of the item $i$, represented by the salient terms of the item, and add it to the Journey Set. %Journey Set $\gets$ Journey Set + Journey^{new}$\}$} 
% \EndIf
% \EndFor

% %\If{$N$ is even}
% %    \State $X \gets X \times X$
% %    \State $N \gets \frac{N}{2}$  \Comment{This is a comment}
% %\ElsIf{$N$ is odd}
% %    \State $y \gets y \times X$
% %    \State $N \gets N - 1$
% %\EndIf
% \State Prune journey clusters with less than $M$ items 
% %\EndWhile
% }
% \end{algorithmic}
% }
% \end{algorithm}
%




% \begin{figure}[!tbp]
% \begin{minipage}{.48\textwidth}
% \begin{algorithm}[H]
% \caption{Infinite Concept Personalized Clustering on One User}
% \label{algorithm:sts}
% \small{
% \begin{algorithmic}
% \Require ${\cal H}_u = \{i_t, t=1, \cdots, T\}$ containing list of items the user interacted with; $\epsilon \in [0, 1]$: salient terms similarity threshold; $c$: Minimum number of items per cluster. Default values: $\epsilon=0.1, c=1$.
% %\Ensure $y = x^n$
% %\State $y \gets 1$
% %\State $X \gets x$
% %\State $N \gets n$
% %\While{user $u$}

% %\State $\text{Journey}_1 = \{i_1\}$
% %\State first item $i_1$
% %\State $\text{Journey}_1 = \{i_1\}$; Journey Set = $\{\text{Journey}_1\}$
% \State Journey Set ${\cal S}_J = \emptyset$ 
% %\While{item $i \in$ Interaction History $H$ of user $u$}
% \For{$t = 1, \cdots, T$}
% %\For{journey $J \in {\cal S}_J$} 
% \State $\forall J \in {\cal S}_J$, compute ItemJourneySim($i_t, J$)  % $\gets$ Cosine similarity between item $i$ and journey $J$
% %\EndFor
% \State $J^\ast$ $\gets$ $\arg\max_{J'\in {\cal J}}$ ItemJourneySim($i_t, J'$) 
% \If{ItemJourneySim($J^\ast$, $i$) $\ge \epsilon$}
% \State {$J^\ast = J^\ast \cup \{i_t\}$} 
% \Else{}
% \State {Start a new journey $J_{\text{new}} = \{i_t\}$, ${\cal S}_J = {\cal S}_J\cup \{J_{\text{new}}\}$. %Journey Set $\gets$ Journey Set + Journey^{new}$\}$} 
% \EndIf
% \State Update the journey representation based on the added item.
% \EndFor

% %\If{$N$ is even}
% %    \State $X \gets X \times X$
% %    \State $N \gets \frac{N}{2}$  \Comment{This is a comment}
% %\ElsIf{$N$ is odd}
% %    \State $y \gets y \times X$
% %    \State $N \gets N - 1$
% %\EndIf
% \State Prune journey clusters with less than $c$ items 
% %\EndWhile
% }
% \end{algorithmic}
% \end{algorithm}
%         %\includegraphics[width=0.9\textwidth]{images/journey_clustering_update.png}
%         %\includegraphics[width=0.9\textwidth]{images/journey_clustering_update.png}
%         %\caption{Journey Clustering Update \minminc{might be better to write it in pseudo-code, and make sure to reflect the sequence aspect of the interactions.
%         %alalama +1 - Fig 1 already provides a visual cue for journey extraction}}
%         %\label{fig:journey_clustering}
% \end{minipage}
% \quad
% \begin{minipage}{.47\textwidth}
%         %\centering
%         %\includegraphics[width=\textwidth]{images/journey_viz_names.png}
%         %\includegraphics[width=0.9\textwidth]{images/woodworking journey viz 1}
%         \includegraphics[width=\textwidth]{images/video_game_strategy_viz.png}
%         \caption{Visualization of journeys across users, with each point representing an extracted and named journey. We generate embeddings for each journey name through Universal Sentence Encoder \cite{cer2018universal} and cluster them with UMAP \cite{mcinnes2018umap}. Highlighted, a \emph{video game strategy} journey and its nearest neighbors in the embedding space, per cosine similarity.%\minminc{the annotation here are using salient terms, is it better to use llm generated names?} %Visualization of journeys across users, with each bubble representing an extracted infinite concepts journey. We generate embeddings through Universal Sentence Encoder \cite{cer2018universal} for the top 5 terms of each journey with at least 5 items and cluster them with UMAP \cite{mcinnes2018umap}. Highlighted, a journey with terms [hacks, woodworking, wood, garden, gardening] and its nearest neighbors in the embedding space, per cosine similarity.
%         }
%         \label{fig:journey_visualization}
%     \end{minipage}%
% \end{figure}


==> Paper_ Extracting and Naming User Journeys for Companion Recommenders (3)/method_naming.tex <==
Once we have extracted journey clusters for a user, we describe each journey in natural language so that it is explainable, scrutable, and controllable \cite{balog2019transparent}. %we want to make them interpretable and use natural language to reason through them. 
This is where Large Language Models (LLMs) come into play. Here, we describe the underlying models we leverage (Section \ref{subsec:models}) and how we adapt them to the domain of user interest journeys (Section \ref{subsec:alignllms}) to capture nuanced natural language descriptions.

\subsubsection{Models}
\label{subsec:models}
In this paper, we build on LaMDa \cite{thoppilan2022lamda} and PaLM \cite{chowdhery2022palm} family of LLMs.%, as well as their instruction-tuned counterparts \kc{adjust based on the results we'll include. e.g., PaLM chilla, GPT}. 

\textbf{LaMDA} \cite{thoppilan2022lamda}, aka. Language Models for Dialog Applications, is a family of Transformer-based, decoder-only, neural language models specialized for dialog, which have up to 137B parameters and are pre-trained on 1.56T words of public dialog data and web text. The models have shown state of the art performance across tasks, including the BigBENCH \cite{srivastava2022imitation}, and have been fine-tuned on human rewrites so to provide safe, interesting, sensible, and specific dialog responses. %\kc{Check to see if indeed our models. alalama: note there is no FLAN version of LaMDA}

 \textbf{PaLM} \cite{chowdhery2022palm}, aka. Pathways Language Model, is a densely-activated decoder-only transformer language model trained using Pathways \cite{barham2022pathways}, a large-scale ML accelerator orchestration system that enables highly efficient training across TPU pods. At the time of release, PaLM 540B achieved breakthrough performance on a suite of multi-step reasoning tasks \cite{chowdhery2022palm}. Its training corpus consists of 780 billion tokens representing a mixture of webpages, Wikipedia articles, source code, social media conversations, news articles and books \cite{chowdhery2022palm}. %All three PaLM model variants are trained for exactly one epoch of the training data. We refer to [14, 19, 80] for more details on the training corpus. 
 
Although we mainly build on LaMDA and PaLM, in our experiments we also considered \textbf{Flan-PaLM}, i.e., the instruction-tuned counterpart introduced by Wei et al.\cite{wei2022finetuned}. This pre-trained model was fine-tuned on datasets where each example is prefixed with some combination of instructions and/or few-shot exemplars, and was shown in \cite{chung2022scaling} to outperform PaLM on several benchmarks. We also considered \textbf{PaLMChilla}, i.e., a PaLM variant trained on an additional data mixture that follows the Chinchilla compute-optimal training procedure \cite{hoffmann2022training} approach.%--- a compute-optimal training procedure, proposing for every doubling of model size the number of training tokens should also be doubled. 

%\textbf{Flan-PaLM.} In addition to the baseline PaLM models, we also considered the instruction-tuned counterpart
%introduced by Wei et al.\cite{wei2022finetuned}. These models are trained using instruction tuning, i.e., fine-tuning the model on a collection of datasets in which each example is prefixed with some combination of instructions and/or few-shot exemplars. In particular, Chung et al. \cite{chung2022scaling} have shown that Flan-PaLM reaches state of the art performance on several benchmarks, outperforming baseline PaLM.  In this study we considered both the PaLM and Flan-PaLM model variants. 

% \textbf{PaLMChilla} is a PaLM variant trained on an additional data mixture that follows the Chinchilla\cite{hoffmann2022training} approach. Chinchilla is the compute-optimal training procedure, proposing for every doubling of model size the number of training tokens should also be doubled. 

\subsubsection{Prompting LLMs for user interest journeys}
\label{subsec:alignllms}
Although general-purpose LLMs have reached state of the art performance on a wide variety of tasks on challenging benchmarks \cite{wang2020superglue}, for them to have good performance for the domain of user journey understanding, it is necessary to align them using domain-specific data. %There are two main approaches for transfer learning and domain adaptation: 
%\begin{enumerate}
% \item \textbf{end-to-end finetuning} of the model with large amounts of in-domain data.
% \item data-efficient alignment techniques building on \textbf{(2a) few-shot prompting} \cite{} and \textbf{(2b) prompt-tuning} \cite{}.
% \end{enumerate}
We explore data-efficient techniques of \textbf{few-shot prompting} \cite{brown2020language} and \textbf{prompt-tuning} \cite{lester2021power}, and data-rich \textbf{end-to-end fine-tuning} \cite{ziegler2020finetuning}.% of the model with large amounts of in-domain data.

\textbf{Few-shot prompting} 
Brown et al. \cite{brown2020language} demonstrated that LLMs are strong few-shot learners. Fast in-context learning can be achieved through including a handful of demonstration examples as prompts in the input context, \emph{without any gradient updates or fine-tuning}. In this study we focused on standard zero-shot, and few-shot. % as discussed below, and we leave chain-of-thought \cite{}, self-consistency \cite{} and least-to-most prompting \cite{} as future work. 
\emph{Zero-shot prompting} queries these models with an instruction describing the task without any additional examples, i.e., \emph{Summarize my interest journey in a concise and interesting way}. 
In \emph{few-shot prompting}, the prompt further includes few-shot examples describing the task through text-based demonstrations. These demonstrations are encoded as input-output pairs. %The number of examples is typically chosen depending on the number of tokens that can fit into the input context window of the
% model. % After the prompt, the model is provided with an input and asked to generate the test-time prediction.   

\textbf{Prompt tuning} \cite{lester2021power} has been proposed as a data efficient domain adaption technique for LLMs. The key idea is that instead of changing \emph{all} model parameters, only a small subset of parameters corresponding to the prompt embedding will be updated given a small training set of input-output pairs (in the order of tens to hundreds). This can be viewed as a soft prompt, as opposed to the hard prompt encoded in few-shot prompting. %The data set size, number of training steps, learning rate, prompt embedding initialization vector, and soft prompt size, all affect the quality of outputs at inference time.

\textbf{Fine-tuning} \cite{ziegler2020finetuning} updates \emph{all} model parameters to adapt to the new domain given a large amount of in-domain data. %This is the preferred prompting strategy 
% Fine-tuning is preferred when there are available domain examples in the order of thousands, and computational cost, or maintaining different models per domain is not a concern. 
Typically, fine-tuning can achieve the best in-domain results with in-domain data in the order of thousands, but is also the most costly in compute and maintenance. An advantage of prompt-tuning compared with fine-tuning, is that the same underlying model (with  same parameters) can be adapted to different domains by using prompt embeddings tuned on the domain data.
 
 To be consistent across prompting strategies,  we pre-processed input-output examples to follow the same format, as shown in Table \ref{tab:format_examples}. % Here we discuss the three approaches in decreasing order of amount of data needed, and amount of model parameter changes.

% ORIGINAL TABLE
% \begin{table}[]
%     \centering
%     \begin{tabular}{|c|c|}
%     \hline
%         input & output \\
%         \hline
%         I watched content with titles: \{ \}. I would describe one of my interests as: &
%         hydroponic gardening \\ %woodworking \minminc{could this example output be too generic}. \\
%         \hline
%     \end{tabular}
%     \caption{Format of input examples across all prompting strategies.}
%     \label{tab:format_examples}
% \end{table}

\begin{table}
\small{
    \centering
    %\newcolumntype{w}{X}
    \newcolumntype{s}{>{\hsize=.5\hsize}X}
    \newcommand{\heading}[1]{\multicolumn{1}{c}{#1}}
    \renewcommand*{\arraystretch}{1.2}
    \begin{tabularx}{\textwidth}{XXs} %{| X | X | X |}
    \toprule
        Prompt Template & Input & Output \\
        \midrule
        I consumed content with titles: \{ \}.\newline I would describe one of my interests as: &
        Natural \& Cultural Heritage Conservation in the Philippine Seas; Seafaring Vessels of Ancient Filipinos; %Philippine Boatbuilding Technology from Balangay to Galleon; 
        The Philippines as a Maritime Nation: Opportunities and Challenges &
        Philippine \newline Maritime History \\
        %Two-Angle Bisectors; Equal Angles; Olympiad Geometry Problem \#99: Cyclic Quad; Equal Segment; Circumcircles &
        %Olympiad Geometry \\
        \hline
        titles: \{ \} interest\_journey: &
        Two-Angle Bisectors; Equal Angles; Cyclic Quad; Equal Segment; Circumcircles &
        Olympiad Geometry \\ \hline
        %Natural \& Cultural Heritage Conservation in the Philippine Seas; Seafaring Vessels of Ancient Filipinos; Philippine Boatbuilding Technology from Balangay to Galleon; The Philippines as a Maritime Nation: Opportunities and Challenges &
        %Philippine Maritime History \\
        %\hline
        keywords: \{ \} interest\_journey: &
        history, microwave, nerd, nostalgia, mp3 %\newline technology, mp3, nostalgia nerd,\newline keyboard, evolution, mp3 player &
        & Evolution of Personal Technology \\
        \bottomrule
    \end{tabularx}
    \caption{Prompt formats: (a) natural language titles prompt, used across all prompting strategies unless stated otherwise; (b) structured titles prompt; (c) structured playlist infinite concepts prompt.
    }
    \label{tab:format_examples}
    }
\end{table}

%Brown et al. [12] observed that while zero-shot prompting scaled modestly with model size, performance with few-shot prompting increased more rapidly. Further, Wei et al. [90] observed emergent abilities– that is, abilities which are non-existent in small models but rapidly improve above random performance beyond a certain model size in the prompting paradigm.

 \subsubsection{Data for aligning LLMs to user journeys}
 \label{subsec:data_alignment}
 To align LLMs to a new domain, it is important to have high-quality examples from that domain. Different prompting techniques, as discussed above, require different volumes of data. % Furthermore, given that our domain of user interest journeys is newly considered, it requires from us being creative in the data we can use as proxy for our domain. Ideally, the data we would like is ones where users while pursuing different interest journeys on the platform, also name themselves in a nuanced way the journeys they pursue. However, we don't have access to that.
The ideal dataset for our task is derived from asking users to annotate and describe interest journeys they are pursuing on the platform in a nuanced and interesting way. This is, however, difficult and time-consuming to achieve at scale. 

\textbf{Fine-tuning data.} To overcome the challenge, we rely on user-curated playlists on the platform as proxy datasets. Each playlist maps groups of content about the same topic to a user-provided name. We only include playlists that have high episodicity (items tend to be consumed in a sequential order) and are classified as learning-focused by a neural network  trained on raters data. We refer to this dataset as \textbf{learning playlists}. The upside is that there are a lot of learning playlists readily available to fine-tune the model (we used twenty thousands examples); the downside is that the ground-truth playlist names tend to be short and noisy, without necessarily the nuanced nature we are looking for.

\textbf{Prompt tuning data.} Prompt tuning requires much fewer examples compared to fine-tuning. High-quality data, however, is crucial to ensure accurate results. Thus, instead of relying on the noisy learning playlists, we curated three small data sources for prompt tuning our models: (D1) \textbf{user interviews}, (D2) \textbf{user collections}, (D3) \textbf{expert-curated collections}, all in the order of less than a hundred examples. The (D1) source is the closest approximation to the ideal dataset, which is collected during our user interviews. We asked 50 users to describe journeys they pursued on the platform for more than a month, and pick from their interaction history the items that helped them toward these journeys. % tries to do as close of an approximation of our user interest domain as possible, i.e., asking in user interviews 50 \kc{adapt} users what is one interest they've pursued in the platform for more than a month; and asking them to provide some item interactions that helped them towards pursuing that interest. 
Source (D2) uses data from a separate platform anchored towards long-term aspirational journeys, where users save items in collections 
%\kc{Can we say it's Keen?} 
that they annotate with collection names.  %and can potentially share with other users. 
Lastly, (D3) comes from learning editorial collections, where expert editors have curated collections of items tailored to learning topics, and have named them in a nuanced and interesting way.

\textbf{Few-shot examples} For few-shot prompting, we only need a handful of examples (five to ten) from the domain of user interest journeys. For consistency, we sample examples from one of the above mentioned prompt tuning data.


%However, since we don't have access to this, we create a proxy domain task of users creating playlists of items and naming the playlists correspondingly. We only limit these to playlists . Note that this is a rough approximation of our task. Users are not prompted to collect playlists to represent their interests. Instead we convert user behavior to a close approximation of our domain task. The downside of this is that the names given by users tend to be on the shorter and more noisy side, without necessarily representing an accurate or interesting summarization of the input. We post-process the input, output examples from this dataset with the prompt formulation described in Table \ref{tab:format_examples}, and then tune all model parameters based on this data.  


 
% \begin{itemize}
%     \item \textbf{user interviews}: asked 70 \kc{adapt} users what is one interest they've pursued in the platform for more than a month; and along with providing some item interactions that helped them towards pursuing that interest. Although these collected examples are the most suitable for the domain, in practice the users provided interest names might be quite noisy, and their provided input can be misaligned with the output.
%     \item \textbf{user collections}: users as part of interacting with a platform save items around a certain topic in a collection, and then give the collection a name. The platform we used was by definition purposed towards long-term interests, so although users were not instructed to provide which items helped them towards their interest, that's exactly what they do. However, there are two key points: (1) interest names are given by users so they might be in a higher or lower granularity than what we want to capture; (2) these were collected in a different platform compared to the one where we evaluate the quality of extracted journey names, so there is some domain shift.
%     \item \textbf{expert-curated collections}: in a learning-specific part of the recommender platform, editors have curated collections of items based on aspirational/learning topics, and have also given names to them. We observed names are the most high quality across the three datasets as they are written by experts who know how to write accurate and interesting names. Again, this data is not from the exact domain of describing interest journeys, but as we'll see in Figure \ref{}, prompt tuning based on them does successful transfer learning.
% \end{itemize}



%\begin{table}[]
%    \centering
%    \begin{tabular}{|c|c|c|}
%        \hline
%         Data& Description & Size  \\ \hline
%         Expert curated collections & &  \\
%         User curated collections & &\\
%         User Interviews & &\\ 
%         \hline
%    \end{tabular}
%    \caption{Data considered during prompt-tuning LLMs for journey name generation. \kc{consider removing if repetitive}}
%    \label{tab:prompt_tuning_data}
%\end{table}

  

%\subsubsection*{Instruction Tuning} Wei et al. \cite{} and Chung et al. \cite{} demonstrated the benefits of multi-task instruction finetuning: the
%Flan-PaLM model achieved state of the performance on several benchmarks such as BIG-bench [47] and
%MMLU [29]. The key principle of Flan is the one of learning to follow instructions where the model parameters are fine-tuned based on data that contain instructions / descriptions of the task to be performed. 
%\kc{How are we constructing examples here?}

%\subsubsection*{Combination of prompting strategies} There have also been successful examples in the literature combing different prompting techniques, such as "hard-soft hybrid prompt tuning" \cite{}. We also find that for the case of PaLM, first prompt-tuning the LLM, and then conditioning the inference on few-shot examples significantly outperforms prompt-tuning alone. \kc{double check! see what about comparison with few shot!}
%, alongside existing techniques that insert hard anchor tokens into a
%soft prompt [53], insert learned soft tokens into a hard prompt [28], or use a learned soft prompt as a prefix
%for a short zero-shot hard prompt [26, 96] 

%\subsubsection{Prompt-tuning for journey naming}

%\kc{
%- Add figure on prompt tuning (fixed model, learn about )
%Which metadata?
%How to construct the prompt 
%On curating small high-quality datasets
%On constructing the prompt 
%Reducing the serving of the model via distillation
%}

%\subsection{Evaluating quality of trained model}


%\subsection{Using prompted models to infer name for extracted journeys}

%Describe how we do so. Including the prompt. 

%Add examples 
%\subsubsection{How to evaluate?}
%Ideally, we want to capture how well 
%Measure the degree to which such models can capture well input in the output


%\subsection{Putting everything together}
%\kc{adapt}





==> Paper_ Extracting and Naming User Journeys for Companion Recommenders (3)/methods.tex <==
%\kc{We need to shrink this whole section, while at the same time providing key details to help reader understand the algorithm.}
The journey extraction component maps a user's overall history into coherent journey clusters. %, where each one has all the relevant contents on one particular deep interest. This effectively translates the problem into a \emph{clustering} one. 
% Thus, the question is how do we cluster the data to obtain journeys? We start with our key hypothesis on which ground our journey extraction approach. 
The most straight-forward approach is to partition the entire item corpus into clusters, where each cluster represents one journey cluster. The caveat is that a single item can often cover multiple nuanced journeys. For example, an item on ``cooking with herbs for improved mental clarity'' can be a part of a ``Mediterranean cooking journey", ``improve your gut health" journey or ``grow your herbs garden journey". A global clustering would then mix these more nuanced journeys together. 
As suggested by our user research, although there are commonalities among user journeys, there are no two identical journeys across users. We thus hypothesize that
%\begin{hyp}%[H\ref{hyp:first}] \label{hyp:first}
\emph{a personalized view of journeys is more appropriate than assuming space of journeys is global}, and propose an infinite concept personalized clustering algorithm.
%\end{hyp}

%This hypothesis is already validated by our user research. Although there should indeed be commonalities among user journeys, how journeys manifest and evolve are highly personal. As an example, a content on "cooking with herbs for improved mental clarity" can be part of very different journeys for different users: a Mediterranean cooking journey for one, vs improve your mental health journey for another. % user, or a grow your herbs garden journey. 
% As a result, a global clustering of all items into a canonical set of journeys might be sub-optimal. To further test this, we will compare our personalized approach with global baselines. 


%The non-personalized view suggests there is a common space of canonical user journeys, and each content item can belong to a journey. Although there should indeed be commonalities among user journeys, how journeys manifest and evolve are highly personal. I.e., a certain content item on "cooking with herbs for improved mental clarity" can be a part of quite different journeys: a Mediterranean cooking journey, improve your gut health journey, or a grow your herbs garden journey. 




%\begin{hyp}[H\ref{hyp:third}] \label{hyp:third}
%\emph{Learning user journeys separately from the recommendation policy is preferred compared to concurrently, for modularity and interpretability purposes.}
%\end{hyp}

%With recent modeling advances, one option would be for the same model that recommends what to show next, also to perform a discovery of the journeys. This is relevant to macro-actions in the hierarchical reinforcement learning literature \cite{} and connects to introducing attention mechanisms to attend to user history \cite{}. Although we think this is a promising direction, it does not satisfy our design goal of interpretability. Another benefit of an in-stages approach is modularity; allowing for plug-and-play of different journey extraction methods, which can in turn accelerate journey-related research. 


%\subsubsection{Personalized vs. Non-personalized}
%The non-personalized view suggests that the space of possible journeys is global. This means there is a common space of canonical user journeys, and each content item can belong to a journey. However, we argue that the same content can be part of different journeys for different users. For example, a certain content item on "cooking with herbs for improved mental clarity" can be a part of quite different journeys: A Mediterranean cooking journey, improve your gut health journey, grow your herbs garden journey, and so on. However, this is not to say that users have no common journeys.
%Rather, how journeys manifest and evolve and which interactions to cluster is a function of the user and their history of interactions so far. We argue the personalized view is more appropriate here: an item interaction's assignment to a journey depends on the user. 
%and which interactions to cluster is a function of the user and their history of interactions so far


%%non-personalized) The space of journeys is global, and if we are to introduce new clustering it should be mapping each video to a cluster based on most likely journey it belongs to. We can find the affinity of the user to a cluster. 
%%(personalized) The assignment of a watch to a cluster will be different depending on the user. This is related to co-clustering ideas as pointed out by Alex Beutel. Or, we can do clustering of watches per user, (e.g., based on salient-terms). 

 %we will explain why we propose to learn users' journeys from scratch while relying on content understanding. 

%\subsubsection{Learned concurrently with planning, or in stages. }

%%%explicit vs. Latent 

%%% Bayesian View Each item has a certain probability of belonging to a journey. It can be related to a certain journey for a user, and another journey for another user.

%\begin{center}
%\begin{table*}
%\footnotesize{}{
%\begin{tabular}{|c| c c c c c c c c|} 
% \hline
 %Entity for journeys & Coherence & Granularity & Recall & Precision & Intra-journey  & Journey-Items  & Interpretability & Cardinality \\ [0.5ex] 
 %\hline\hline
%Topic Annotations: Semantic & NA & varying & low & high & NA  & NA & \checkmark & high\\
% \hline
%Topic Annotations: Taxonomic & $\times$ & coarse & low & low & NA & NA & \checkmark & \checkmark \\
% \hline
%Co-Occurrence-based Topic Clusters & $\times$ & coarse & low & low & $\times$ & $\times$ & $\times$ & \checkmark \\
% \hline
%Multi modal similarity-based Topic Clusters & \checkmark & fine-grained & medium & high & $\times$ & $\times$ & $\times$ & $\times$ \\ 
% \hline
%Infinite concepts- personalized clustering & \checkmark & right& high & high & \checkmark & \checkmark& \checkmark & \checkmark \\ 
% \hline
%\end{tabular}}
%\caption{Comparison of various entities for clustering watch histories into journeys.}
%\label{table:1}
%\end{table*}
%\end{center}





%WatchEmbed clusters (not available yet)
%Experts on clustering Yifat Amir, and the team believe based on prior work on learning clusters that watchembed based clusters might be what we need to achieve semantic coherence. This is pending on the availability of infra. 

%\subsubsection{Proposed Algorithm: Infinite Concept Personalized Clustering}
\label{subsec:personalized_clustering}
%\subsubsection*{Background} 
%\label{subsec:infinite_concepts}
%\kc{help from yifat}

%entire cluster, by aggregating the salient terms of the items in the same journey cluster.
%One can then represent a list of items similarly by aggregating the sets of salient terms of the items with their salient score ... \minminc{is infinite concept equivalent to salient term? I thought one infinite concept is a combination of multiple salient terms. If so, detail it out.}

%The terms are learned via a supervised machine learning model, learning to score how important the terms are for the concept being described.  

% \subsubsection*{Key Insights}
% \begin{itemize}
%     \item Salient terms is a universal embedding space where different types of concepts can be represented. Thus, so can journeys. I.e., we can obtain the salient terms representation of the entire cluster, by aggregating the salient terms of the items in the same journey cluster.
%     \item Cosine similarity between the salient terms of two concepts measures the overlap between the two. Given that we want the resulting journey clusters to be thematically coherent, we can use cosine similarity among salient terms embedding as the measure of thematic coherence. This dictates the clustering update for when an item from user's interaction history should be added to the journey cluster, and how new clusters are being formed. 
% \end{itemize}

% \subsubsection*{Clustering Update}
% \begin{itemize}
%     \item When the salient terms representation of an item from user's interaction history  has high cosine similarity with the representation of a journey cluster, it should be added to this cluster. Otherwise, a new cluster is created.
% \end{itemize} 

%An illustration of our algorithm is shown in Figure \ref{fig:journey_clustering}. 

% \begin{wrapfigure}{l}{0.5\textwidth}
% \begin{minipage}{0.48\textwidth}
% \vspace{-0.1in}
% \begin{algorithm}[H]
% \SetAlgoLined
% \begin{singlespace}
% \caption{Infinite Concept Personalized Clustering on a User}
% \label{algorithm:sts}
% \begin{algorithmic}
% \small
% \textbf{Input:} ${\cal H}_u = \{i_t, t=1, \cdots, T\}$ containing list of items the user interacted with; $\epsilon \in [0, 1]$: salient terms similarity threshold; $c$: Minimum number of items per cluster. Default values: $\epsilon=0.1, c=1$. \\
% \textbf{Initialize:} Journey Set ${\cal S}_J = \emptyset$ \\
% \For{$t = 1, \cdots, T$} {
% $\forall J \in {\cal S}_J$, compute ItemJourneySim($i_t, J$)  \\
% $J^\ast$ $\gets$ $\arg\max_{J'\in {\cal J}}$ ItemJourneySim($i_t, J'$) \\
% \uIf{ItemJourneySim($J^\ast$, $i$) $\ge \epsilon$} {
% $J^\ast = J^\ast \cup \{i_t\}$
% } 
% \Else{
% Start a new journey $J_{\text{new}} = \{i_t\}$, ${\cal S}_J = {\cal S}_J\cup \{J_{\text{new}}\}$. 
% }
% Update the journey representation based on the added item.\\
% }
% Prune journey clusters with less than $c$ items 
% %\EndWhile
% \end{algorithmic}
% \end{singlespace}
% \end{algorithm}
% \end{minipage}
% \end{wrapfigure}


\begin{figure}
\begin{minipage}{0.48\textwidth}
\begin{algorithm}[H]
\SetAlgoLined
\begin{singlespace}
\caption{Infinite Concept Personalized Clustering (ICPC) on a User}
\label{algorithm:sts}
\begin{algorithmic}
\small
\Statex \textbf{Input:} ${\mathcal H}_u = \{i_t, t=1, \cdots, T\}$ containing list of items the user interacted with; $\epsilon \in [0, 1]$: salient terms similarity threshold; $c$: Minimum number of items per cluster. Default values: $\epsilon=0.1, c=1$. 
\State \textbf{Initialize:} Journey Set ${\mathcal S}_J = \emptyset$ 
\State \For{$t = 1, \cdots, T$} {
$\forall J \in {\mathcal S}_J$, compute ItemJourneySim($i_t, J$)  \\
$J^\ast$ $\gets$ $\arg\max_{J'\in {\mathcal J}}$ ItemJourneySim($i_t, J'$) \\
\uIf{ItemJourneySim($J^\ast$, $i$) $\ge \epsilon$} {
$J^\ast = J^\ast \cup \{i_t\}$
} 
\Else{
Start a new journey $J_{\text{new}} = \{i_t\}$, ${\mathcal S}_J = {\mathcal S}_J\cup \{J_{\text{new}}\}$. 
}
Update the journey representation based on the added item.\\
}
\State Prune journey clusters with less than $c$ items 
%\EndWhile
\end{algorithmic}
\end{singlespace}
\end{algorithm}
\end{minipage}
\quad\quad
\begin{minipage}{.45\textwidth}
\vspace{-0.1in}
        \includegraphics[width=\textwidth]{images/video_game_strategy_viz.png}
        \caption{Visualization of journeys across users, with each point representing an extracted and named journey. We generate embeddings for each journey name through Universal Sentence Encoder \cite{cer2018universal} and cluster them with UMAP \cite{mcinnes2020umap}. Highlighted, a \emph{video game strategy} journey and its nearest neighbors in the embedding space, per cosine similarity.%\minminc{the annotation here are using salient terms, is it better to use llm generated names?} %Visualization of journeys across users, with each bubble representing an extracted infinite concepts journey. We generate embeddings through Universal Sentence Encoder \cite{cer2018universal} for the top 5 terms of each journey with at least 5 items and cluster them with UMAP \cite{mcinnes2018umap}. Highlighted, a journey with terms [hacks, woodworking, wood, garden, gardening] and its nearest neighbors in the embedding space, per cosine similarity.
        }
        \label{fig:journey_visualization}
    \end{minipage}%
\end{figure}

% \begin{wrapfigure}{l}{0.5\textwidth}
% \begin{minipage}{0.48\textwidth}
% \vspace{-0.3in}
% \begin{algorithm}[H]
% \begin{singlespace}
% \caption{Infinite Concept Personalized Clustering on A User}
% \label{algorithm:sts}
% \begin{algorithmic}
% \small
% \Require ${\cal H}_u = \{i_t, t=1, \cdots, T\}$ containing list of items the user interacted with; $\epsilon \in [0, 1]$: salient terms similarity threshold; $c$: Minimum number of items per cluster. Default values: $\epsilon=0.1, c=1$.
% \State Journey Set ${\cal S}_J = \emptyset$ 
% \For{$t = 1, \cdots, T$}
% \State $\forall J \in {\cal S}_J$, compute ItemJourneySim($i_t, J$)  % 
% \State $J^\ast$ $\gets$ $\arg\max_{J'\in {\cal J}}$ ItemJourneySim($i_t, J'$) 
% \If{ItemJourneySim($J^\ast$, $i$) $\ge \epsilon$}
% \State {$J^\ast = J^\ast \cup \{i_t\}$} 
% \Else{}
% \State {Start a new journey $J_{\text{new}} = \{i_t\}$, ${\cal S}_J = {\cal S}_J\cup \{J_{\text{new}}\}$. 
% \EndIf
% \State Update the journey representation based on the added item.
% \EndFor
% \State Prune journey clusters with less than $c$ items 
% %\EndWhile
% \end{algorithmic}
% \end{singlespace}
% \end{algorithm}
% \end{minipage}
% \end{wrapfigure}

\textbf{Infinite concepts.} We start with annotating each item with a set of  salient terms (unigrams and bi-grams), each with an associated weight called salience score \cite{37686, gamon2016identifying}. Sources for the unigrams and bigrams are the text (e.g., title, description) of the item, search query that lead to clicks on the item, anchor text, and so on. Together these terms provide the semantic meaning of the item. The salience score of each term is always between $[0, 1]$, which is obtained by training a supervised learning model to predict human ratings of relevance between the salient term and the item, with tf/idf demotions built in. One can then obtain the salient term representation of a group of items by aggregating salient terms of individual items, taking into account their salience score, resulting in a new set of salient terms representing the item group. This way, any group of items (or any concept for that matter) can be represented in the salient term space, which can be thought of as an infinite dimension embedding space where one salient term represents one dimension. Furthermore, the similarity between any two concepts can be computed in terms of cosine similarity of the salient terms embeddings, measuring the overlap of salient terms.

\textbf{Infinite Concept Personalized clustering (ICPC).} As depicted in Algorithm 1%Figure~\ref{fig:journey_clustering} 
%~\ref{algorithm:journey_extraction}
%\minminc{a pseudo-code will be really helpful}
, our proposed algorithm effectively performs online clustering of a user's interaction history, based on the salient terms of the comprising items. Each user starts with an empty journey cluster set. We parse the user historical interactions one by one, each time assigning an item to the nearest, in terms of salient terms cosine similarity, journey cluster. Meanwhile, the representation of the assigned cluster is updated with the salient terms and salience scores of the newly assigned item. If no cluster is nearby (determined by thresholding the cosine similarity), a new cluster is created with the item assigned to it. The algorithm outputs the  resulting journey clusters, which by definition will be thematically coherent, as shown in figure~\ref{fig:journey_visualization}. The highlighted journey, extracted and named as ``video game strategy" is closest to journeys such as ``video game walkthroughs" and ``game AI". %As a result, each user journey cluster is represented using the infinite concepts described above with salient terms and scores. 

% We refer to these combined approaches as infinite concepts personalized clustering (ICPC).
% with the journey clusters being updated on the fly. Every time an item gets assigned to the nearest journey cluster, that cluster's representation is updated with the new assigned item. If no cluster is nearby, to preserve the thematic coherence of the journey clusters, a new cluster is created with that item assigned to it. Given the expansive and continuous nature of salient terms, we refer to journeys extracted via our approach as "infinite concepts" journeys.

%\begin{figure}
%    \centering
%    \includegraphics[scale=0.3]{images/journey_clustering_update.png}
%    \caption{Illustration of our proposed personalised journey extraction algorithm.}
%    \label{fig:journey_clustering}
%\end{figure}

%Thus, our algorithm is going over the items from a user's interaction history. 
%What is even more interesting is we can interpret salient terms as a universal embedding space, where by aggregating salient terms across items we can represent in the salient term space any concept or any content group. %There are three parameters that control the aggregated terms, and their corresponding salience: power mean, salience power, and number of accumulated terms. The power in the power mean can control how max-ish or min-ish is the accumulation. A power higher than 1.0 will result in an aggregated 0.8 term higher than two 0.4 terms, whereas a power of 1.0 behaves like a weighted arithmetic average.  If you want a 0.8 term higher than two 0.4,  will do that. A power of 1.0 behaves like a weighted arithmetic average.
%\kc{I am not sure best way to explain them unless I expose the aggregation formula.} 
%\kc{alalama: I'm only referencing the similarity threshold in the results. maybe we can mention num acc terms, since other parameters don't make as big of a difference } 



%Via salient terms aggregation functions every YT entity besides video (e.g., clusters, channels, users) can be represented in the salient term space, which gives us the added benefits of enabling exploration of relevant journeys, and other concepts (e.g., clusters/channels/legos in the same salient terms space). 


%we can represent user journeys in the salient term space. The way the aggregation of salient terms across items happens is via 
%is we can aggregate item salient terms to create salient terms for content groups, e.g., content creators, or topics. And this way, we can compare any concept represented in the infinite dimension salient term space with any other concept, using cosine similarity between the two.

%What is quite interesting about salient terms is that it can be seen as an infinite dimension space, in which every concept, including items, topics, creators, and so on, can be represented in.

%Since any concept can be represented in the salient terms space, so can journeys. 

%\subsubsection{Proposed Algorithm*}
%\kc{Add here the picture.}
%Returning to our user journey setting, we expand on how we can extract user journeys from the user history by leveraging salient terms. Our approach relies on three core ideas:
%\begin{itemize}
%    \item At any point, a user is either resuming an existing journey or starting a new one.
%    \item A journey is a sequence of user-item interactions, all coherent around a particular theme. 
%    \item We can aggregate salient terms across items of the journey to represent user journeys in the infinite concept space.
%\end{itemize}

%Given that besides items, journeys can also have a salient term representation, each item of the user interaction history can be compared with each discovered journey in terms of cosine similarity between salient terms. 


%\begin{algorithm}
%\caption{Journey Extraction via Salient Terms for User $u$ \kc{perhaps better to include the figure instead of this table?}}\label{alg:cap}
%\label{algorithm:sts}
%\small{
%\begin{algorithmic}
%\Require salient terms similarity threshold $T: [0, 1]$; interaction history H comprised of items $i$ of user $u$; $M$: Minimum number of items per cluster. Default values: $T=0.1, M=1$.
%\Ensure $y = x^n$
%\State $y \gets 1$
%\State $X \gets x$
%\State $N \gets n$
%\While{user $u$}

%\State $\text{Journey}_1 = \{i_1\}$
%\State first item $i_1$
%\State $\text{Journey}_1 = \{i_1\}$; Journey Set = $\{\text{Journey}_1\}$ 
%\While{item $i \in$ Interaction History $H$ of user $u$}
%\For{item $i \in$ Interaction History $H$ of user $u$}
%\For{journey $j$ in Journey Set} 
%\State ItemJourneySim($i, j$) $\gets$ Cosine similarity between item $i$ and journey $j$
%\EndFor
%\State $j^\ast$ $\gets$ $\arg\max_{j'\in \text{Journey Set}}$ ItemJourneySim($j'$, $i$) 
%\If{ItemJourneySim($j^\ast$, $i$)>= T}
%\State {Add item $i$ to the journey, and update journey's salient term representation, based on salient terms of item $i$.} 
%\Else{}
%\State {Start a new journey composed of the item $i$, represented by the salient terms of the item, and add it to the Journey Set. %Journey Set $\gets$ Journey Set + Journey^{new}$\}$} 
%\EndIf
%\EndFor

%\If{$N$ is even}
%    \State $X \gets X \times X$
%    \State $N \gets \frac{N}{2}$  \Comment{This is a comment}
%\ElsIf{$N$ is odd}
%    \State $y \gets y \times X$
%    \State $N \gets N - 1$
%\EndIf
%\State Prune journey clusters with less than $M$ items 
%\EndWhile
%}
%\end{algorithmic}
%}
%\end{algorithm}
%

%\begin{figure*}[!h]
%  \includegraphics[width=1.0\textwidth]{images/125 - pizza oven.png}
%  \caption{Visual representation of a "building a pizza oven" journey, extracted by the infinite concepts method. \kc{There is also a singleton on bed frame. Perhaps with different threshold it could be removed?}}
%  \label{fig:sts_journey}
%\end{figure*}



%Although salient terms on their own cannot be taken as sub-journeys (varying granularity, infinite cardinality etc.), we can utilize cosine similarity among salient terms associated with the items of the interaction history, as a way to segment the user history into journeys. 

%based on online personalized clustering of interactions

%\subsubsection{How the proposed approach is designed to preserve journey desiderata}
%By representing journeys in the infinite space of concepts, we gain many of the desirerata specified in Section \ref{sec:journey_service}. Given that only items with larger than a threshold $T$ salient term similarity will be added to a journey cluster, by definition extracted clusters should have high thematic coherence. 




==> Paper_ Extracting and Naming User Journeys for Companion Recommenders (3)/metrics_methods.tex <==
 \subsection{Desiderata}
\label{subsec:desired_properties}
\kc{Consider moving to metrics section}
%Reiterating from Section \ref{sec:formulation}, we want to assist long-term journeys that involve multi-step explorations of interest/topics people want to spend more time on. % and expect to engage with for more than a month. 
%For this, we argue the need for a service mapping for each user their overall history (lifelong journey) into possible journeys. %(Figure \ref{fig:journey_pictorial}). 


%from the user history sequences of items that should be all about the same interest journey. 
%come up with a splitting of the lifelong history of the user to sequences, where each sequence covers the above properties. 
%We first specify our design goals, which will largely guide the desired properties for the extracted journey clusters. %When designing a service  mapping each user's  overall history into possible journeys, the goals we have for the expected improvements will largely guide the design. 
The goals of journey extraction are two-fold:
\begin{enumerate}
    \item[(D1)] Enable better recommendation quality and user experience
    \item[(D2)] Enable better organization of content by journeys
\end{enumerate}
%\subsection{Desiderata for journey entity extraction}
\label{sec:desiderata}
We specify the desired properties for the extracted journeys:
%To reflect the above design goals, . %This way we can inform whether existing metadata grouping content are a good fit for journeys, and prescribe the preferred approach to extract journeys.  
% and its applications. 
%\begin{figure}
%  \includegraphics[width=0.5\textwidth]{images/sequence.png}
%  \includegraphics[width=0.5\textwidth]{images/sequence2.png}
%  \caption{Identify that the user is on two journeys: the blue and the red one. A crucial decision is based on which metadata / representation we should decide what is red and what is blue? Because if we look at too high of a level (less granular) red and blue might be merged into one single sub-journey. And if we look too low of a level more granular, we might end up with multiple shades of blue and multiple shades of red, whereas in reality it's just two journeys we need to support well: blue and red.  }
%  \label{fig:journey_pictorial}
%\end{figure}
%\begin{itemize}

    \noindent \textbf{Thematic coherence/ High Precision:} Each extracted journey should only contain items about the same thematic need; %it shouldn't contain items from other journeys. 
    \begin{equation}
        \text{Precision} = \frac{\text{\# of well retrieved journey items in the cluster}}{\text{\# items in the extracted cluster}}
    \end{equation}%which preserve the thematic coherence of the journey; it shouldn't contain items from other journeys
    %When a journey is about another semantic meaning it should be pulled apart into another journey. E.g., "learning the ukulele" is a different journey from "learning the guitar".
    \noindent \textbf{High Recall:} Each extracted journey should ideally retrieve all related items from the user history which are a part of the same journey. %Can be viewed as high coverage, i.e., covering all items/concepts which should be a part of the journey.
    \begin{equation}
        \text{Recall} = \frac{\text{\# of well retrieved journey items in the cluster}}{\text{\# items in the ground-truth journey}}
    \end{equation}
    \noindent \textbf{Right granularity:} %The extracted journeys should be neither too general (e.g., "learn music"), nor too specific (e.g, "learn A, B, C chords on ukulele"), but rather at the right granularity (e.g., “learn the ukulele”), to be useful. 
    The extracted journeys should neither be too general, nor too specific to be useful for changing the recommendations accordingly. Finding the right  granularity is challenging, it however does manifest in the precision and recall tradeoff---when too coarse, many journeys will be unnecessarily merged, thus increasing recall while deteriorating precision; When too fine-grained, precision will be increased (at its limit each interaction is a separate journey), but recall will suffer. 
    %Measuring granularity is hard; thus, it can be indirectly measured via having both high coherence and high recall.
    
    Other metrics that can be used as proxies for granularity evaluation are %\textbf{cardinality-related metrics}, including 
    \begin{itemize}
        \item \textbf{\# of journey clusters per user}: based on our user research, most users pursue 1-3 interest journeys; thus more clusters per user could point to too fine-grained clusters; 
        \item \textbf{\# items per journey cluster}: clusters with too few items can hardly justify as long-term journey, as this should span multiple interactions.
    \end{itemize} 
    By definition we will be eliminating clusters with only one-item, thus other proxy  metrics are:
    \begin{itemize}
        \item \textbf{\# unclustered items per user}, and
        \item \textbf{\# users without journey clusters}.
    \end{itemize}
%    Especially the \# of journey clusters per user can reveal whether too many journeys are extracted, as from our user research we know that the majority of users at a point in time pursue 1-3 interest journeys. Also, a cluster with just a couple of items can hardly justify as long-term interest journey, spanning multiple interactions.
%\begin{equation}
%\textbf{Cardinality} = \text{Total \# of Extracted Journeys per user}
%\end{equation}, 
%\begin{equation}
%\textbf{Per-journey Cluster Cardinality} = \text{\# of Clusters per journey}
%\end{equation}, 
%\begin{equation}
%    \textbf{Documents }
%\end{equation}
%    as well as not too many journeys
    % Granularity affects precision and recall/coherence. When too coarse, many journeys will be merged into one by the method, thus increasing recall but resulting in poor precision. When too fine-grained, precision will be perfect (at it's limit each item is a separate journey), but recall will suffer. It also affects cardinality, as too granular clusters will lead to more journeys. Minimizing cardinality though is not an objective on its own, as this will 
% Measuring granularity is hard; thus, it can be indirectly measured via having both high coherence and high recall, as well as not too many journeys. Another way to indirectly measure it is via the number of items belonging to a cluster, as too many clusters consisting of too few items would probably mean poor granularity, and . Mean # clusters per journey. 
%    I.e., we want the journeys to be at the granularity of “learn the ukulele”; not “learn A, B, C chords on ukulele”, but also not “learn a musical instrument”. Too granular of journeys might end up containing only a handful of items, and too broad of journeys might merge too many unrelated journeys together. Either fallback would minimise the benefits of journey extraction.
%    \item \textbf{High Precision}: Each of the journeys should contain only items which preserve the thematic coherence of the journey; it shouldn't contain items from other journeys.
    \noindent \textbf{Intra-Journey connectivity} and \textbf{Item/Metadata <> Journey connectivity}: The extracted journeys should reflect the \emph{structure} among items belonging to them, and the structure among journeys.
%    Related  journeys should live close together in the semantic/embedding space, so that related journeys can be explored \cite{}.
%    \noindent \textbf{Comparability of journeys <> items / content metadata:} Ability to represent journeys in the same space as items, and as other metadata, to allow user exploration across different entity types.

    \noindent \textbf{Interpretability:} Each journey should have an associated label, or set of concepts describing what the journey is about. %This will facilitate the content organization by journeys design goal.
%    \item \textbf{Low Cardinality:} Related to the right granularity property, at every point every user is typically on journeys in the order of tens, not more. This is also crucial to control the complexity introduced when including journeys  to adapt recommendations.
%\end{itemize}

% Structure between content items, and among journeys, as in being able to compare , and visualizing the key concepts each journey is about.  
% 

%https://docs.google.com/document/d/118klhbcOr1Kz2EekJjrRyiubr1z7xVAUXkyQ1-AOG_k/edit?resourcekey=0-ktyTB8oqKuNB4Fe2ktLZJQ#heading=h.b1ku1ghop8on

\subsubsection*{How desiderata satisfy the design goals:} We argue that the properties of thematic coherence, high recall, and right granularity are very important for both design goals. Imagine a journey extracted at too fine granularity of "A, B, C chords"; or of low coherence containing irrelevant items into a high-valued journey; or of low recall not realizing that user interactions span the same journey. This could hardly result in an improved user experience, or good content organization. Furthermore, the ability to express items, content metadata, and journeys in the same space, can enable the recommender to find items tailored to the journey, and allow user explore related journeys as well---both crucial for a good recommendation experience (D1). The ability to interpret what the journey is about in human readable format can allow the system explain to users content recommendation through the lens of interest journeys, and if right, have the users feel understood (D2). %that the system gets what their interest journeys are.  will feel that the system understands what their real-life goals are, and the bigger interest arcs they are pursuing

%E.g., imagine a journey being extracted at the level of <A, B, C> chords. 

%\subsubsection{Enable better recommendation quality and user experience} 
%Our main goal is to improve the recommendation quality, and the user experience. The hypothesis is that conditioning the recommendations on the journey that the user is on will both allow the model to better figure out the recommendations they can give, and in the process give the user more journey-aware recommendations. The ability to express both items and journeys in the same space can allow for finding items which are a good match. Also, the ability to explore related journeys, and express in the same space other content entities (such as creators, genres, and so on) can enable better user exploration allowing users to traverse the content space much more effectively. Furthermore, being able to extract the journeys at the right granularity is important, where each extracted journey is all about the same longer-term interest, and it's neither too broad nor too specific. 

%\subsubsection{Enable better organization of content by journeys}
%We want to better organize the abundance of potential content to recommend to user by their journeys. This way, the users 
%\begin{enumerate}
%    \item will feel that the system understands what their real-life goals are, and the bigger interest arcs they are pursuing;
%    \item will find easier what they are looking for related to their interests, and be able to better control their  experience. 
%\end{enumerate}
%This is related to explaining to users why they see certain content through the lens of long-term user journeys, and giving them control as to whether they continue pursue certain long-term interests or not. 
%Thus, being able to explain to users why they see certain content through the lens of long-term user journeys, as expressed in natural language, is important.
%being able to explain journeys through concepts in natural language space is important. %Note that this goal can be seen as rather a means to achieve even more effectively the first goal of improved user experience. 


==> Paper_ Extracting and Naming User Journeys for Companion Recommenders (3)/results.tex <==
%\kc{Initial draft: Alberto}
% Results: https://colab.corp.google.com/drive/1d-XQ_F1E1GDcsgbxAGHQEBaOgF1nvZNJ?resourcekey=0-MkmyxECd2JeIN8fNpO6X6w#scrollTo=lYHxObTkcb1N

%The following section describes the results of journey extraction methods on a large-scale content recommendation platform.


%\subsection{Analysis of Journey Extraction Results}
\subsection{Experimental Setup}
\label{subsec:analysis}
%\subsubsection*{Annotation \& Evaluation Challenges.}
%To compute quantitative metrics such as precision and recall, we need someone annotating histories with what should be the right journeys. This is an extremely difficult task. Thus, we rely on qualitative measures of thematic coherence, and granularity; as well as quantitative evaluation of the proxy metrics for granularity as explained in Section \ref{subsec:desired_properties}, which in turn affect precision and recall.

%To facilitate the qualitative comparisons, we built a visual tool to display and compare journey extraction methods, as shown in Figure \ref{fig:visual_journeys}. Together, combining the insights from the qualitative and quantitative comparisons, we can get a full picture of the quality of extracted journeys.


%Before we introduce our evaluation settings, it is worth highlighting the challenges of evaluating the quality of extracted journeys, especially in terms of their granularity.  
%When extracting journeys on real user histories (experimental setup E1), we can only evaluate resulting clusters qualitatively (for which we built a visual tool as shown in Figure \ref{fig:visual_journeys} to facilitate comparisons), and quantitatively only in terms of proxy metrics for granularity. However, in order to compute metrics of precision and recall, which affect granularity, we would need someone to label each example in the resulting cluster to verify that all retrieved items are about the same theme (precision) and also someone to annotate each item of user histories with the  "right"/"golden" journeys it should be split into (recall). We argue that  while precision/thematic coherence is relatively easier to evaluate qualitatively by verifying all retrieved items are about the same theme, computing recall is considerably harder. From experience, we found that to annotate by hand just a couple of users histories takes a lot of time, as it requires consuming each item in the first place to understand what it is about. That's why we introduce experimental setup E2 as well of using proxy ground-truth/ golden journeys. 
%In the previous evaluation setup, we focused on qualitative evaluation of extracted journey clusters, together with quantitative comparison in terms of proxy metrics for right granularity. Here, we argue that  while precision/thematic coherence is relatively easier to evaluate qualitatively by verifying all retrieved items are about the same theme, computing recall is considerably harder. Computing recall 

\textbf{Metrics.} As discussed in Section~\ref{sec:method:overview}, measuring the right granularity of the extracted journey is extremely challenging. We look at qualitative results when extracting journeys on real user histories (evaluation data E1 explained below). Figure \ref{fig:visual_journeys} shows one comparison between journeys extracted using different methods. To obtain quantitative results comparing different journey extraction algorithms, we measure \emph{precision} (percentage of items correctly assigned the right journey cluster) and \emph{recall} (percentage of items belonging to each journey cluster getting retrieved) on a ``golden journey'' set detailed in the following (evaluation data E2). 

\textbf{Evaluation Data} We created two evaluation sets to evaluate journey extraction: 
\begin{enumerate}
    \item[E1] \textbf{Unlabeled Histories:} 300 user interaction histories, each with at least 10 valued interactions over 30 days, resulting in a dataset of 18,370 user-item interactions. %An item consists of a title, description, language, content, image thumbnail, and author. 
    % We define a meaningful user-item interaction as one that the user engaged with for at least three minutes. Additionally, we select user-item interactions with a predicted long-term satisfaction score in the top percentiles, based on aggregated user surveys. To facilitate qualitative analysis, we restrict our analysis to items in the English language. The 300 user histories have a median length of 31.5, a mean length of 61.23 and a standard deviation of 69.41. The longest one contains 479 items; the smallest, 11. 
    We define a valued user-item interaction as one where 1) the user engaged with at least $X$ minutes, and 2) a model that predicts user satisfaction surveys has found that the predicted user satisfaction score is in the top percentiles. The 300 user histories have a median length of 31.5, a mean length of 61.23 and a standard deviation of 69.41. The longest one contains 479 items; the shortest, 11.
    \item[E2] \textbf{Learning playlists as golden journeys:} %Existing collections of items satisfying the key properties we care about: users interact with items in the collection sequentially, and  the items are around the same theme/ user need. For this, we leveraged user-curated collections, of saved content items of the platform into collections. We made sure to only use collections with: (i) \emph{high episodicity}, so to satisfy the constraint that the items are likely to be consumed one after the other in order; (ii) \emph{ten items or more}, so to satisfy the condition that "deep interest spanning multiple interactions"; (iii) content items about learning new skills, satisfying the "valued interest journey" concept, as learning was one of the key categories of valued content revealed from our user study. We ended up with 5,000 such collections, which we use as golden journeys, comprised in total of 130,381 items.  Each such collection can be thought of as one user with one journey, with the goal of the algorithm to group all items into the same cluster. To evaluate algorithm's capability to differentiate different journeys and not just produce one cluster putting everything together, we also consider a two golden journeys per user setup introducing some noise. For each collection, we also give to  the algorithm another random collection as its pair as well, and run the extraction algorithm on top; we ideally want the method to group the items into the right two journeys. %Here, we want to further test in a similar quantitative set up of 5,000 user-curated collections as above, whether on a per-user basis with multiple journeys the algorithm can correctly split the union of the journeys's items into the right journey clusters. To set this up, for each user-curated collection, .  
    %the algorithm's task is to see if it can extract all items into the same cluster (preferred), or whether it will split them into multiple journey clusters.
    We sampled 5,000 learning playlists as explained in Section~\ref{subsec:data_alignment} as the golden journeys, comprised in total of 130,381 items. For each user we randomly sample and mix two playlists/journeys, and the goal is to cluster the items back into the two playlists.
    %two experiment setups: 1) each user has a single journey (playlist), and the goal is to cluster all the items into a single cluster; 2) 
    %each user has two playlists/journeys randomly sampled and mixed together, and the goal is to cluster items back into the two playlists.  %\minminc{I wonder if it is less confusing to only talk about the two-journey setup. Removing the one-journey from Table 2 as well.}
%To evaluate the journey extraction algorithms we rely on cardinality metrics:
\end{enumerate}

%\subsubsection{Baseline:  Predefined Global Groupings}
%\label{subsec:baseline}
\textbf{Baselines.} We compared with baseline approaches that uses different strategies to partition the entire item corpus into non-personalized global clusters; each cluster then becomes one journey cluster: %We outline the two baseline approaches that are typically used to partition the item corpus into groups in large-scale recommender systems. These predefined groupings globally clustering content items into clusters are a non-personalized way to group user histories into journeys.
%We describe two baseline approaches using predefined groupings to group user histories into journeys. % They both are pre-defined groupings, globally clustering all content items into clusters, and represent the state-of-the-art of content groupings in our  industrial recommenders.

%Here, we explore alternative content metadata we can use to associate content with journeys. Following the categorization of the design choices above, these metadata are non-personalized (global clustering of the corpus based on content attributes and/or global user behavior patterns), predefined (e.g., every item is already associated with each of these clusters) and in-stages (they are not learned co-currently with recommendation policy). 


%Here, we explore alternative content metadata we can use as a way to associate content with journeys. Following the categorization of the design choices above, these metadata are non-personalized (global clustering of the corpus based on content attributes, and/or global user behavior patterns), predefined (e.g., every item is  associated already with each of these clusters) and in-stages (they are not learned co-currently with recommendation policy). 


%\subsubsection{Topic Annotations: Semantic}

%A topic annotation is the relationship from an item to an entity from the Knowledge Graph. The annotation, which is supposed to describe what the item is about, can be seen as an edge between two nodes in a bipartite graph (items  on one side, and semantic entities on the other side), and can contain the edge score.
%The semantic annotations are supposed to describe what the item is about. 
%Each item is associated with multiple semantic annotations, of varying granularity and of varying confidence level, with the highest confidence annotation not necessarily being the one of the finest/coarsest granularity. This makes semantic annotations unfit to capture journeys, as all extracted journeys should have the same desired granularity; thus, we exclude them from our results. %Thus, this cannot satisfy the right granularity property, and we omit it from experiment results comparison. 

%\subsubsection{Topic Annotations: Taxonomic}
%Taxonomic  annotations classify items in a taxonomy of a few thousands broad semantic entities, which are supposed to give a high-level category of the item. The taxonomy is hierarchical, with three levels. Top level nodes are for instance Music, Gaming, Entertainment, etc. Each of them is then refined into a variety of music genres, game genres, etc. We found that the third level of the hierarchy is the closest to what we might be interested in for journey extraction, as the top two levels would be too generic. Nevertheless, even the third level still seemed too coarse of granularity (e.g., the ukulele and the guitar learning journey being merged into one). We also found that the predefined entities overly focus on certain types of journeys (music) compared to others. This leads us to exclude taxonomic annotation from our  baselines of journey extraction, as not all journeys can be expressed in the predefined taxonomy, and at the right level. %Since this metadata would force many journeys to belong in the same generic annotation, we omit it from result section too.

\begin{enumerate}
    \item \textbf{Clusters based on co-occurence behavior}. A topic cluster for each item is produced by: 1) taking the item co-occurrence matrix, where entry (i, j) counts the number of times item i and j were interacted with by the same user consecutively; 2) performing matrix factorization to generate one
embedding for each item; 3) using k-means to cluster the learned embeddings into $K$ clusters; 4) assigning each item to the nearest cluster centroid.% based on item embedding.
    \item \textbf{Clusters based on multimodal item similarity} These clusters group items together based on their audiovisual similarity, using online agglomerative/hierarchical clustering. The first-level of the hierarchy is capturing the macro-clusters, while the second level contains items all of fixed distance $\epsilon$; each macro cluster would then serve as a journey cluster. Online clustering works by comparing each new item with the micro-clusters in terms of embedding similarity, and assigns it to the closest micro-cluster. If too often an item is found in close proximity to multiple micro-clusters, micro-clusters are merged.
\end{enumerate}


\textbf{Parameters.} For the proposed Infinite Concept Personalized Clustering (we will refer to it here as \emph{ICPC} for brevity), we set the similarity threshold parameter to 0.1 unless explicitly stated otherwise, as we found qualitatively that this results in the most coherent journeys of the right granularity. For the baselines, we used parameters as tuned in a large-scale production recommender system. For the co-occurrence based topic clusters, the total number of clusters $K$ is 10,000; for multi-modal similarity-based clusters, the distance $\epsilon$ is set to 70. For all methods, we prune resulting clusters with a single item (we specify when we prune those with less than 5 items). %We omit from candidate journey extraction methods topic annotation methods, as neither satisfies the right granularity property, and as such, it'd be unfair to compare. 



%\subsubsection*{Metrics.} To compute quantitative metrics such as precision and recall, we need someone annotating histories with what should be the right journeys. This is an extremely difficult task. Thus, we rely on qualitative measures of thematic coherence, and granularity; as well as quantitative evaluation of the proxy metrics for granularity as explained in Section \ref{subsec:desired_properties}, which in turn affect precision and recall. %cardinalities, that can serve as proxy metrics for granularity, in turn affecting precision and recall as discussed in Section \ref{subsec:desired_properties}. 

%\subsection*{Qualitative Comparison}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.95\textwidth]{images/112_sts.png}
    \begin{minipage}{\textwidth}
    \centering
    \includegraphics[width=0.475\textwidth]{images/112_swarm.png}
    \includegraphics[width=0.475\textwidth]{images/112_mm.png}
    \end{minipage}
    \hfill
    % \begin{minipage}{0.49\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{images/112 - swarm.png}
    %     \includegraphics[width=\textwidth]{images/112 - mm.png}
    % \label{fig:sim_threshold}          
    % \end{minipage}
    \caption{Visual depiction of an infinite concepts personalized clusters journey extraction for \emph{surfing}. Shown at the top, the journey's salient terms representation. Below, the set of documents with a thumbnail and title for each. In contrast, multi-modal similarity topic clusters journeys only retrieve 6 documents, and co-occurrence topic clusters split these into 2 clusters, each with 2 documents.}
  \label{fig:visual_journeys}
  \vspace{-0.2in}
\end{figure}

% ORIGINAL PICS
% \begin{figure}[!t]
%     \centering
%     \begin{minipage}{0.45\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{images/112 - sts.png}
%   \includegraphics[width=\textwidth]{images/112 - swarm.png}
%   \includegraphics[width=\textwidth]{images/112 - mm.png}
%   \caption{Visual representation of journey extraction methods for a "surfing" journey. Each extraction method is displayed with the journey representation as string, the number of items per journey and a list of items with metadata. Top: Infinite terms extraction produces the largest journey. Middle: multi-modal similarity topic clusters extraction includes a subset of the infinite terms journeys; unclustered items not shown. Bottom: co-occurrence topic clusters extraction splits the journey into two; unclustered items not shown. \minminc{show in table instead, figure is not readable. print it and check.}}
%   \label{fig:visual_journeys}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{.45\textwidth}
%         \centering
%             \includegraphics[width=0.9\textwidth]{images/110 - sts 0.1.png}
%  % \end{minipage}
%   \caption{Increasing similarity threshold to 0.1 extracts two additional journeys: \textit{London public transportation}, \textit{transportation video games}  (unclustered items not shown), compared to only one \textit{public transportation} journey retrieved when threshold is set to 0.05, comprised of the union of shown items. \minminc{consider remove this figure if short on space} \minminc{figure not readable, summarize in table instead.}} % Visual representation comparison of infinite terms journey extractions varying the similarity threshold. Left: similarity threshold set to 0.05 produces one \textit{public transportation} journey. Right: similarity threshold set to 0.1 extracts two additional journeys: \textit{London public transportation}, \textit{transportation video games}  (unclustered videos not shown). }%\kc{K: Interestingly, I am not sure which one might be the best one. Should we comment on that? A: included an additional journey and added an interpretation below}}
%   \label{fig:sim_threshold}
%     \end{minipage}
% \end{figure}

%\begin{figure}
%  \includegraphics[scale=0.21]{images/112 - sts.png}
%  \includegraphics[scale=0.21]{images/112 - swarm.png}
%  \includegraphics[scale=0.21]{images/112 - mm.png}
%  \caption{Visual representation of journey extraction methods for a "surfing" journey. Each extraction method is displayed with the journey representation as string, the number of items per journey and a list of items with metadata. Top: Infinite terms extraction produces the largest journey. Middle: multi-modal similarity topic clusters extraction includes a subset of the infinite terms journeys; unclustered items not shown. Bottom: co-occurrence topic clusters extraction splits the journey into two; unclustered items not shown.}
%  \label{fig:visual_journeys}
%\end{figure}



%\begin{table}
%\footnotesize{}{
%\begin{tabular}{|p{2cm}| p{1.1cm}|p{1.1cm}|p{1cm}|p{2cm}|p{1.5cm}|p{1cm}}
% \hline
% Journey Extraction Method & \# journeys per user & \# journeys per user\newline $\geq 5$ items & \# items per journey & \% un-clustered items per user & \# users without journeys \\
% \hline
%Co-Occurrence-based\newline Topic Clusters & mean: 7.18\newline std: 7.35 & mean: 1.95\newline std: 2.64 & mean: 4.32\newline std: 4.87 &  79.55\% & 8 \\
% \hline
%Multi modal similarity-based Topic Clusters & mean: 4.07\newline std: 5.85 & mean: 0.58\newline std: 1.38 & mean: 3.38\newline std: 3.51 & 90.27\% & 73 \\ 
% \hline
%Infinite concepts\newline(similarity\_thr=0.1) & mean: 7.80\newline std: 7.50 &  mean: 3.40\newline std: 3.71 & mean: 6.92\newline std: 9.65 & 43.45\% & 0 \\ 
% \hline
%Infinite concepts\newline(similarity\_thr=0.2) & mean: 9.37\newline std: 9.87 & mean: 2.79\newline std: 3.61 & mean: 4.91\newline std: 6.25 & 58.99\% & 1 \\ 
% \hline
%\end{tabular}}
%\caption{Quantitative evaluation across journey extraction methods in terms of proxy granularity metrics.} % \kc{Same here: Seems thr 0.2 gives 9.37 mean vs 7.80 total >1 doc journeys. A: this is expected, note that #docs/journey goes down with higher sim --> more fragmented journeys with higher sim }}
%\label{table:extraction_stats_per_user}
%\end{table}

%\begin{figure}[!t]
%    \centering
    %\includegraphics[width=0.33\textwidth]{images/dense_items_journeys.png}
    %\includegraphics[width=0.33\textwidth]{images/journeys_per_user.png}
    %\includegraphics[width=0.33\textwidth]{images/perc_unclustered_items.png}
    %\includegraphics[width=0.33\textwidth]{images/journey_length.png.png}
    %\caption{Quantitative evaluation across journey extraction methods in terms of proxy granularity metrics.}
    %\label{fig:extraction_stats_per_user}
%\end{figure}

\subsection{Key Results}
% Here we examine the quality of the extracted journeys using our proposed ICPC algorithm and baselines from both qualitative and quantitative comparisons  across the two experimental setups.% , we can get a full picture of the quality of extracted journeys.
%\begin{minipage}{\textwidth}
%\centering
%\includegraphics[width=\textwidth]{images/Proxy granularity metrics (1).png}
%\label{fig:extraction_stats_per_user}
%\caption{Comparison of journey extraction methods across proxy granularity metrics in (E1) setup.}
%\end{minipage}
\begin{figure}%{l}{0.45\textwidth}
\vspace{-0.3in}
\includegraphics[width=0.45\textwidth]{images/Proxy_granularity_metrics_1.png}
\caption{\textbf{Comparison of journey extraction methods across proxy granularity metrics in (E1) setup.}}
\label{fig:extraction_stats_per_user}
\vspace{-0.1in}
\end{figure}Here we qualitatively and quantitatively compare the extracted journeys using our proposed ICPC algorithm and baselines across the two experimental setups.




\subsubsection*{ICPC achieves long coherent journeys, and is more robust to trivial coherence as obtained by singleton journey clusters.}
\label{subsec:docs_per_journey}
%From our qualitative review of infinite concepts extracted journeys, we conclude that most journeys with at least 5 items are thematically coherent.
As shown in Figure~\ref{fig:visual_journeys} and Figure \ref{fig:extraction_stats_per_user}, the proposed method produces longer coherent journeys than baselines. %Furthermore, we find our method to be relatively robust to the journey granularity controlled by the salient term similarity threshold. Lowering the similarity threshold to 0.05 still produces coherent journeys. %the resulting coherence is tolerant to changes in granularity as controlled by the salient term similarity threshold. Journey clusters are coherent even when setting similarity threshold as low as 0.05.  Trivial coherence can be obtained in the topic cluster methods due to sparsity of documents per journey cluster (Table \ref{table:extraction_stats_per_user}). That is, since most extracted journeys contain a single document, they can be trivially thematically coherent within themselves. 
The baselines on the other hand tend to produce trivially coherent journeys by assigning each item to a different cluster. 
Figure \ref{fig:extraction_stats_per_user} shows that a fraction of 0.79 of items per user are singletons for the co-occurrence based baseline; the number increases to 0.90 for the multi-modal similarity-based ones. This fraction is much lower, but exists for our method too ($\sim0.4$). 


% Item relationships in infinite terms space can be harnessed through the similarity threshold parameter, which provides a certain degree of control in journey granularity. Figure \ref{fig:visual_journeys} shows a recurring pattern across extraction methods: infinite concepts-based journeys outperform global topic clusters in extracting journeys at the right semantic granularity.  %\kc{Which threshold did we use here?}. 
% Since topic clusters are predefined, their semantic granularity is defined by  co-occurrence and multi-modal similarity metrics, which may not capture long-term interests. In the surfing example journey, multi-modal topic cluster journeys have smaller recall with respect to infinite concepts journeys. Co-occurrence topic cluster journeys are extracted at a granularity below the semantics of surfing, leading to poor recall; the same journey cluster should capture the entirety of the surfing journey, instead of being split into multiple journeys with no further semantic refinement. 



%\begin{figure}[!tbp]
%  \centering
%  \begin{minipage}[b]{0.45\textwidth}
%    \includegraphics[width=\textwidth, left]{images/110 - sts 0.05.png}
%  \end{minipage}
 % \hfill
%  \begin{minipage}[b]{0.45\textwidth}
%    \includegraphics[width=0.45\textwidth, right]{images/110 - sts 0.1.png}
 % \end{minipage}
%  \caption{Increasing similarity threshold to 0.1 extracts two additional journeys: \textit{London public transportation}, \textit{transportation video games}  (unclustered items not shown), compared to only one \textit{public transportation} journey retrieved when threshold is set to 0.05, comprised of the union of shown items.} % Visual representation comparison of infinite terms journey extractions varying the similarity threshold. Left: similarity threshold set to 0.05 produces one \textit{public transportation} journey. Right: similarity threshold set to 0.1 extracts two additional journeys: \textit{London public transportation}, \textit{transportation video games}  (unclustered videos not shown). }%\kc{K: Interestingly, I am not sure which one might be the best one. Should we comment on that? A: included an additional journey and added an interpretation below}}
%  \label{fig:sim_threshold}
%\end{figure}



%Not only does journey granularity increase with a higher similarity threshold, but so does does document precision with respect to the journeys' thematic and semantic specificity. 

%\subsection*{Quantitative Comparison}

\subsubsection*{ICPC %retrieve the longest, most dense, coherent journeys, while 
corroborates our user research findings that each user pursues a few journeys.}
%From Figure \ref{fig:visual_journeys} and from our overall qualitative evaluations, our method can retrieve the longest journeys, while being coherent. We confirmed this quantitatively too via the proxy metrics, as shown in Table \ref{table:extraction_stats_per_user}. We find:
%\begin{enumerate}
    %\item 
   % (1) In terms of \textbf{\# items per journey} (column 3),  infinite concepts method extracts more items per journey on average, albeit with the highest variance. Conversely, multi-modal similarity extracts the least items per journey, and the variance is lower. We summarize this as: \emph{Infinite Concepts Personalized Clusters retrieve the longest coherent journeys.}
  %  \item 
  %  (2) \textbf{\% unclustered items per user} When we restrict the number of items per journey cluster to a minimum of 5 , we notice that most of the topic clusters journey extractions contain under 2 items, which would hardly meet the desired properties of long-term interests. A portion of infinite concepts journeys also suffer from this limitation, but to a significantly smaller extent.
    %\item
    As shown in 
    Figure \ref{fig:extraction_stats_per_user}%Table %\ref{table:extraction_stats_per_user} (column 2 $\#$ journeys $\ge$ 5 items per user)
    , restricting the minimum number of items per journey to a value of 5, i.e., considering only dense journeys, the mean number of journeys per user to significantly decrease. The decrease is very prominent for multi-modal similarity topic clusters, suggesting that clusters are sparser. Conversely, \emph{the cardinality of ICPC clusters and co-occurence topic clusters is consistent with user research} (Section \ref{sec:uxr}), that 7 of out 10 users pursue 1-3 interests simultaneously and 3 of out 10 sustain 4 or more.
    %We summarize this finding as Infinite Terms and Co-Occurrence Topic Cluster journey extractions display cardinalities consistent with user research.
    %\item 
    % (4) \textbf{\# users without journey clusters} We notice that multi-modal topic clusters do a poor job on retrieving all user journeys, given the relatively larger proportion of users for whom no journeys were extracted (73 out of 300). In contrast, infinite concepts personalized clustering results in no users without extracted journeys. %Our approach retrieves 1.74 times more journeys with >=5 documents compared to the co-occurrence-based topic clusters, and 5.82 times more such journeys compared to the multi modal similarity-based topic clusters.
    %\end{enumerate}


%\begin{table*}[!htb]
%    \caption{Global caption}
%    \begin{minipage}{.4\linewidth}
%      \centering
%        \caption{Comparison of extracted journeys vs. golden journeys in (E1) setup.}
%        \label{tab:extraction_stats_playlists}
%        \begin{tabular}{ | c || c | c | c |}
%          \hline
%           & \multicolumn{3}{|c|}{(E1) setup} \\
%           \hline \hline
%           \textbf{Method} & \textbf{\# journeys/user} & \textbf{\# dense journeys/user} & \textbf{\# clusters / journey} \\ \hline
%           Co-occurrence & 0.29 & 106,936 & 4.56 \\ \hline
%           Multi-modal & 0.16 & 71,388 & 3.63 \\ \hline
%           ICPC (\textbf{ours}) & \textbf{0.82} & \textbf{13,488} & \textbf{2.42} \\ 
%           \hline
%    \end{tabular}
%    \end{minipage}
%    \begin{minipage}{.4\linewidth}
%      \centering
%        \caption{Comparison of extracted journeys vs. golden journeys in (E2) setup.}
%        \label{tab:extraction_stats_playlists}
%        \begin{tabular}{ | c || c | c | c |}
%          \hline
           %& \multicolumn{3}{|c|}{Two golden journeys per user} \\
           %\hline \hline
           %\textbf{Method} & \textbf{Recall} & \textbf{\# journeys} & \textbf{\# clusters / journey} \\ \hline
           %Co-occurrence & 0.29 & 106,936 & 4.56 \\ \hline
           %Multi-modal & 0.16 & 71,388 & 3.63 \\ \hline
           %ICPC (\textbf{ours}) & \textbf{0.82} & \textbf{13,488} & \textbf{2.42} \\ 
           %\hline
    %\end{tabular}
    %\end{minipage} 
%\end{table*}

\begin{figure}%5{l}{0.5\textwidth}
%\begin{figure}[]
\centering
%\begin{minipage}{\textwidth}
%\centering
%\includegraphics[width=\textwidth]{images/Proxy granularity metrics (1).png}
%\label{fig:extraction_stats_per_user}
%\caption{Comparison of journey extraction methods across proxy granularity metrics in (E1) setup.}
%\end{minipage}
%\begin{minipage}{\textwidth}
%    \centering
    \small{
    \begin{tabular}{ | c || c | c | c |}
          \hline
           & \multicolumn{3}{|c|}{Two golden journeys per user} \\
           \hline \hline
           \textbf{Method} & \textbf{Recall} & \textbf{\# journeys} & \textbf{\# clusters / journey} \\ \hline
           Co-occurrence & 0.29 & 106,936 & 4.56 \\ \hline
           Multi-modal & 0.16 & 71,388 & 3.63 \\ \hline
           ICPC (\textbf{ours}) & \textbf{0.82} & \textbf{13,488} & \textbf{2.42} \\ 
           \hline
    \end{tabular}
    }
    %\caption{Comparison of extracted journeys vs. golden journeys in (E2) setup.} %\minminc{table 2 and 3 results seem a bit conflicting between co-occurrence and multi-modal, where multi-modal seems to be more specific/fine-grained in table 2, while co-occurrence is more specific in table 3. Might need to explain.}}

%    \end{minipage}
    \caption{\textbf{Comparison of journey extraction methods in E2.}}
    \label{tab:extraction_stats_per_user}
%\end{figure}
\end{figure}
%\end{wrapfigure}



\subsubsection*{ICPC %extracts journeys at the right granularity, which 
can easily control journey granularity via the similarity threshold.}
%Figure \ref{fig:sim_threshold} shows how the similarity threshold parameter affects the extracted journey's granularity. 
We find that at a lower threshold, more items are grouped into the same journey cluster, resulting in a coarser granularity. Increasing the threshold renders a larger number of journeys that are more specific, unearthing deeper semantic relationships between items. For example, in a public transportation-related example journey, we find that a 0.1 similarity threshold breaks up the \textit{public transportation} journey (with 0.05 threshold) into three journeys: a general \textit{public transportation} journey, a more specific \textit{London public transportation} and a \textit{public transportation video game simulations}. With pre-defined global clusters, it is difficult for the baselines to produce journey clusters at different granularity.


%\begin{table}[]
%    \centering
%    \begin{tabular}{ | c || c | c | c | c | c | c |}
%          \hline
%           & \multicolumn{3}{|c|}{One golden journey per user} & \multicolumn{3}{|c|}{Two golden journeys per user} \\
%           \hline \hline
%           \textbf{Method} & \textbf{Recall} & \textbf{\# journeys} & \textbf{\# clusters / journey} & \textbf{Recall} & \textbf{\# journeys} & \textbf{\# clusters / journey} \\ \hline
           %Co-occurrence & 0.61 & 51,377 & 2.22 & 0.29 & 106,936 & 4.56 \\ \hline
           %Multi-modal & 0.73 & 34,780 & 1.78 & 0.16 & 71,388 & 3.63 \\ \hline
           %Infinite concepts \minminc{use consistent name} (\textbf{ours}) & \textbf{0.96} & \textbf{6,749} & \textbf{1.20} & \textbf{0.82} & \textbf{13,488} & \textbf{2.42} \\ 
           %\hline
    %\end{tabular}
    %\caption{Comparison of extracted journeys vs. golden journeys. \minminc{remove one-journey result.} \minminc{add precision metric to two-journey results.}} %\minminc{table 2 and 3 results seem a bit conflicting between co-occurrence and multi-modal, where multi-modal seems to be more specific/fine-grained in table 2, while co-occurrence is more specific in table 3. Might need to explain.}}
    %\label{tab:extraction_stats_playlists}
%\end{table}


%We can see in Table \ref{table:extraction_stats_global} that the infinite concepts method extracts more documents per journey on average, albeit with the highest variance. Conversely, multi-modal similarity extracts the least documents per journey, and the variance is lower. When we restrict the number of documents per journey to a minimum of 5 (column 3 in Table \ref{table:extraction_stats_per_user}), we notice that most of the topic clusters journey extractions contain under 2 documents, which would hardly meet the desired properties of long-term interests. A portion of infinite concepts journeys also suffer from this limitation, but to a significantly smaller extent.

%\subsubsection{Infinite Concepts Personalized Clusters retrieve the most journeys.}
%\kc{A: is this true? can we say something about precision? K: I am not sure, as for recall we ideally need golden set; same for precision. Left is as retrieve, rather than talking about recall.}


%\subsubsection{Infinite Terms and Co-Occurrence Topic Cluster journey extractions display cardinalities consistent with user research.}



% \begin{figure}[b]
%   \includegraphics[width=0.23\textwidth]{images/mean_journeys_per_user@1.png}
%   \includegraphics[width=0.23\textwidth]{images/mean_journeys_per_user@5.png}
%   \caption{Mean number of journeys per user by extraction method. Left: minimum number of videos per journey = 1. Right: minimum number of videos per journey = 5.}
%   \label{fig:mean_journeys_per_user}
% \end{figure}

% \begin{figure}[!t]
%   \includegraphics[width=0.23\textwidth]{images/mean_docs_per_journey.png}
%   \includegraphics[width=0.23\textwidth]{images/unclustered_journeys_frac.png}
%   \caption{Left: mean number of documents per journey by extraction method, excluding single-document journeys. Right: Mean fraction of single-document journeys per user by extraction method.}
%   \label{fig:mean_docs_per_journey}
% \end{figure}




%Looking at number of documents per journey on a user basis in Table \ref{table:extraction_stats_per_user} shows that our method extracts the longest journeys. 

%Based on the number of extracted journeys per user, we conclude that topic clusters, multi-modal and co-occurrence-based, are more sparse than infinite terms personalized clusters. \kc{Does sparse here refer to documents per journey, or journeys per user. Not sure whether this paragraph tries to convey the meaning of the previous paragraph, or a different one.}. While this is not entirely surprising given the discrete nature of topic clusters, it shows promise that the continuous natural language space of infinite terms may capture semantic relationships between documents at a higher granularity.


%\begin{table}
%\footnotesize{}{
%\begin{tabular}{|p{2.25cm}| p{1.25cm}|p{1.25cm}|p{1.25cm}|p{1cm}|}
% \hline
% Journey Extraction Method & Total\newline journeys & Total\newline journeys\newline $\geq 5$ documents  & Documents per journey & Users without journeys  \\ [0.5ex] 
% \hline\hline
%Co-Occurrence-based\newline Topic Clusters & 2,153 & 585 & mean: 4.32\newline std: 4.87  & 8 \\
% \hline
%Multi modal similarity-based Topic Clusters & 1,221 & 175 & mean: 3.38\newline std: 3.51 & 73 \\ 
% \hline
%Infinite concepts\newline(similarity\_thr=0.1) & 2,340 & 1,020 & mean: 6.92\newline std: 9.65 & 0 \\ 
% \hline
%Infinite concepts\newline(similarity\_thr=0.2) & 2,810 & 837 & mean: 4.91\newline std: 6.25 & 1 \\ 
% \hline
%\end{tabular}}
%\caption{Comparison of global journey extraction results.}% \kc{With larger threshold are we not expecting less no of journeys? It looks it's the opposite for the total journeys column 0.1 vs 0.2. A: we expect more journeys with a higher sim bc it's harder for docs to cluster together}}
%\label{table:extraction_stats_global}
%\end{table}



%\subsubsection{Infinite Terms journeys are comparable among themselves.}
%Infinite concepts journeys can be compared semantically through the same similarity measure described in Section 5.3.
%Topic clusters, both multi-modal similarity and co-occurrence,-based journeys can only be compared in a binary fashion; either all of the items in a journey belong to a topic cluster or they do not.
%Similarly, only infinite concepts provides a way to compare journeys and documents, since the infinite concepts representation of journeys is a weighed aggregation of its documents' representation. %\textcolor{red}{If we can add the visualization of nearby journeys that'd be great.} 
%Figure \ref{fig:journey_embedding_viz} demonstrates that infinite terms journeys can be mapped to a continuous natural language space through sentence embeddings with meaningful semantic relationships between journeys.

%\subsubsection{Infinite Terms journeys are accessibly interpretable.}
%Infinite terms is the one journey extraction method that can be accessibly interpreted  without incurring in significant computation costs by examining the item corpus. 




% \subsection{Clusters of overall user journeys}
% How do we represent journeys? Salient terms string? 
% How do we cluster journeys? Kona/USE embeddings + ClustOn?
%   Would be good to use sts similarity as weigths - may be too much work to use with ClustOn.
% Ideally match semantic UXR journey categories/groupings

% NOTES:
% We don't have ground truth journeys to compute recall and precision
% \subsubsection{Recall}
% \subsubsection{Precision}
% TODO(alalama): we don't have an implementation for extracting journeys with Legos
% TODO: Topic annotations - how do we represent Lego journeys?

% DEBUG:
%We report journeys/user and documents/journey cardinality metrics for each extraction method in Figures \ref{fig:mean_journeys_per_user} and \ref{fig:mean_docs_per_journey}.

%\subsubsection{Infinite Concepts Personalized Clusters achieve better precision and recall compared to baselines}. From qualitatively looking at resulting journeys, we find co-occurrence based topic clusters to have poor precision; i.e., a cluster (e.g., about "beginner ukulele") can contain items that should belong to the other journeys (e.g., "learning history of music"). In addition, these clusters have poor recall, i.e., not all items about "beginner ukulele" will be in the same cluster; rather, items belonging to the same journey were found to belong to several clusters. We found multi-modal clusters to perform considerably better for capturing thematic coherence, compared to co-occurrence ones. By definition, all items belonging to the same cluster should be coherent, as they are all very similar visually/acoustically. However, the $\epsilon$ controlling the granularity of the micro-clusters, together with the agglomerative clustering, leads the micro-clusters to be more granular than desired. For example, in a ukulele learning journey, the discovered clusters would be of the type "learn A, B, C" chords, and "learn to play my first song on ukulele", rather than extracting all of them in a "beginner ukuelele learning" journey. As a result, these type of clusters could be suitable for capturing stages of a journey but not entire journeys. %The cardinality of these clusters is in the order of millions, which is another drawback; making journey-aware recommenders with these clusters as proxy for journeys would increase the computational complexity of recommendation.

%By representing journeys in the infinite space of concepts, we gain many of the desired properties we want for journeys. First, by definition of how journey clusters are created, thematic coherence of journey is preserved. Similarly, this allows for high precision (all items in the same cluster are all about the same journey), and high recall (all items which are about the same journey are retrieved into the same cluster). Precision, and Recall, along with the granularity of the journeys, and cardinality of number of journey clusters per user, are effectively controlled via the salient terms similarity threshold; in practice, we found a global threshold of $0.1$ can result in journey clusters of high precision, recall, and the desired granularity (not too coarse, nor too fine-grained). We found on average users are on a handful of journeys, thus preserving the low cardinality property---which can be further controlled via the minimum number of documents per journey (Section \ref{subsec:docs_per_journey}).%; however, for extreme cases we can set a maximum number of journeys per user threshold to further control cardinality.  

%Furthermore, given that all journeys will be expressed in the salient term space, comparability among journeys will be preserved; related journeys will have high cosine similarity. Also, given that both items, and journeys, and other item metadata are all expressed in the same universal embedding space, comparability of journeys to items/content metadata will be possible; this will be important for building journey-aware recommenders to find items which are good fit for journey, and to allow the user explore nearby creators, topics, etc. Finally, given that salient terms describe concepts in terms of important one or two-grams, representing journeys in the salient term space allows for interpretability.

%\textcolor{red}{Iris: Do we expect our audience to understand what infinite concepts mean in this section? if not, maybe we can expand on it? Seems like this is the only place we mention it before chapter 6. Maybe an "in a nutshell, infinite concepts refer to" sentence would help at the end of this section. Alberto: my attempt to connect salient terms & infinite concepts.}

\subsubsection*{ICPC achieves the highest recall.}
%Using the experimental setup (E2), we are able to compute recall, along with other proxy metrics, i.e., total \# of journeys, which ideally should be 5,000 as there is one journey per each of the 5,000 users/collections; mean \# clusters per journey, which should be 1. To compute  recall , when the algorithm extracts multiple clusters per user, we assume the resulting journey cluster from the algorithm is the one containing the most retrieved items, aka. the longest found journey. By definition, since all items belong to the same journey, no matter how the algorithm splits items into clusters, all clusters would have precision 1.
%since there are no interleaved items from wrong journeys, precision is 1. 

%\footnote{This points to conducting research on how to annotate histories with associated journeys; which is an open significant problem, outside the scope of this paper.} 

%From the quantitative and qualitative results above, we observe that infinite concepts personalized clustering leads to the right granularity, to the longest and most dense journeys, and to a good cardinality of journeys, among all considered methods. These together serve as proxy for the desiderata of high recall, high precision, and thematic coherence. However, for further validation of our approach, we want to compute these metrics directly. 



%For each journey/collection, we run the journey extraction algorithms, and computed recall, and cardinality metrics. When a golden journey was split into multiple clusters, we assumed that the extracted journey cluster is the one containing the most retrieved items (the longest found journey). Note that that by definition, precision of all extracted journey clusters is 1, as the items grouped into a cluster will always belong to the golden journey.

%\begin{itemize}
%    \item Recall: Average (\# of well-retrieved journey items in the cluster / \# items in golden cluster)
%    \item Precision: Average (\# of well-retrieved journey items in the cluster / \# items in extracted cluster
%    \item Total \# extracted journey clusters 
%    \item Mean \# clusters per journey 
%\end{itemize}

%achieves almost perfect recall (0.96) in the single playlist setup, being able to group all the items from the same playlist into one cluster. %We see that as well from t
%The mean \# of clusters per journey is close to 1 (1.2); meaning, only a few journeys were split into more clusters. %Also, the total \# of extracted journeys is 6,749 as opposed to the ground truth 5,000 journeys (1.35 times more). 
%\minminc{i saw Kristin also brought up the point on one journey having trivia solution, please make sure to touch on that and explain the two journey mixing is used as an additional validation point.}
%Co-occurrence based topic clusters performed much worse in comparison; recall is considerably lower to 0.61, and 10.28 times more journeys are extracted compared to golden, due to incorrectly splitting the same journey into multiple clusters. Multi-modal similarity based one has similar issues. % This is a direct result from the fact that the same journey is usually split into multiple clusters, on average 2.22. Although multi-modal similarity-based topic clusters are better than co-occurrence ones (recall 0.73; 6.95 more journeys compared to golden), our method considerably outperforms it, too. 
%\begin{table}
%\footnotesize{}{
%\begin{tabular}{|p{3cm}| p{1.3cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% Journey Extraction Method & Recall & Total \# journeys & Mean \# clusters per journey \\ [0.5ex] 
% \hline
%Co-Occurrence-based\newline Topic Clusters & 0.61 & 51,377 & 2.22 \\
% \hline
%Multi modal similarity-based Topic Clusters & 0.73 & 34,780 & 1.78 \\ 
% \hline
%Infinite concepts & 0.96 & 6,749 & 1.20 \\ 
% \hline
%\end{tabular}}
%\caption{Comparison of extracted journeys vs. golden journeys; one golden journey per user.}% \kc{With larger threshold are we not expecting less no of journeys? It looks it's the opposite for the total journeys column 0.1 vs 0.2. A: we expect more journeys with a higher sim bc it's harder for docs to cluster together}}
%\label{table:extraction_stats_playlists}
%\end{table}
%\begin{table}[!t]
%\footnotesize{}{
%\begin{tabular}{|p{3cm}| p{1.3cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% Journey Extraction Method &  Recall & Total \# journeys  & Mean \# clusters per journey \\ [0.5ex] 
% \hline
%Co-Occurrence-based\newline Topic Clusters & 0.29  & 106,936  & 4.56  \\
% \hline
%Multi modal similarity-based Topic Clusters & 0.16  & 71,388  & 3.63  \\ 
% \hline
%Infinite concepts & 0.82  & 13,488 & 2.42 \\ 
% \hline
%\end{tabular}}
%\caption{Comparison of extracted journeys vs. golden journeys; two golden journeys per user.}% \kc{With larger threshold are we not expecting less no of journeys? It looks it's the opposite for the total journeys column 0.1 vs 0.2. A: we expect more journeys with a higher sim bc it's harder for docs to cluster together}}
%\label{table:extraction_stats_playlists_pairs}
%\end{table}
%\textbf{Setup: Two golden journeys per user}
%We also compute the same metrics, in the harder setup of two golden journeys per user, where we interleave another collection's items with the golden collection. %, and ask the method to extract the corresponding journey clusters.  
% To compute the metrics as above, we need to decide for each extracted cluster which of the two golden journeys per user we should compare to; we decide to compare with the one that has the largest intersection of retrieved items. Then, averaging over all of the retrieved clusters, over 5,000 users, we compute the same metrics. 
%Again, because we choose to compare the retrieved cluster with the golden one that it has the largest intersection with we get precision (close to) 1. 
%We observed similar results. % we observe that once more that the Infinite concepts personalized clustering does the best job in extracting the journeys. 
Considering the (E2) setup of two golden journeys/playlists per user, we see from Figure \ref{tab:extraction_stats_per_user} that our ICPC algorithm 
 achieves much higher recall compared with baselines.
On average, 2.42 journey clusters are extracted per user using ICPC; close to the ground truth of 2 journeys per user.  % Our method can also achieve recall 2.83 times better than co-occurrence based topic clusters, and 5.12 times better than multi-modal similarity-based. 
From the total \# of journeys, we see that our method retrieves 1.3 more journey clusters than golden, versus co-occurrence gets around 10.7 more journey clusters. 

Together, our findings suggest that our proposed ICPC approach can effectively cluster noisy interaction histories into journeys with the desired properties, significantly outperforming the non-personalized baselines. % This further confirms our hypothesis that a personalised approach for journey extraction has more merit compared to global canonical user journeys.
%Finally, note that the thematic coherence property was already satisfied in the first golden journeys experiment, as by definition the user-curated collections are all about the same thematic/user need. This is further validated by the fact that our infinite concepts clustering method, which by definition should produce thematically coherent journey clusters, typically retrieves all items into the same one cluster, and does not split it into multiple. For the two-golden journeys per user setup, this thematic coherence of the extracted clusters is not guaranteed, as the extracted clusters could wrongly retrieve items from the "wrong" journey to them. In this case, measuring coherence is effectively reduced into measuring average false positives; items that the algorithm thought are all about the same journey, but they are not. We see from Table \ref{table:extraction_stats_playlists_pairs} that all three methods have false positives close to zero (thus high coherence), with multi-modal having 0 false positives, and our method having the most, although extremely small, 0.038 false positives (again, high coherence). This emphasizes that looking into multiple metrics to evaluate the quality of journey clusters is crucial---we see that recall, together with cardinality (as measured by total number of journeys per user), and granularity (as measured by total number of discovered journeys) can give a very comprehensive view of the quality of journey extraction methods. 



%good granularity and good 
%The above insights of the right gr
% This result, together with the good granularity and thematic coherence results we present in what follows lead us to argue that infinite concepts personalized clustering has the highest recall.
 
%Different properties for resulting extracted journeys can be measured differently. The right granularity property can be evaluated only qualitatively; The properties of interpretability, comparability among journeys, and between journeys-items and interpretability are by construction, and can also be measured easily qualitatively.

%For the properties of high recall, high precision, and thematic coherence, we can see qualitatively how they hold, but would be great to measure quantitatively too. However, measuring them is extremely hard. The reason is that we need to reference them to ground truth ideal journeys. This requires human raters who are able to go through user histories, consisting of many documents, that could range to 479 items, and come up with the "golden" journeys that should be extracted. And then see whether for each journey cluster, all items from the history about one journey are retrieved in the cluster (high recall) and all items in a cluster are all about one journey (high precision). Given that this requires large human labor, we anecdotally look at 10 sampled user histories, and annotate them with golden journeys, and compare journey extraction methods' results to them. \kc{TBD. Measure this, and include results.}


==> Paper_ Extracting and Naming User Journeys for Companion Recommenders (3)/results_naming.tex <==
Next, we evaluate the quality of journey naming in describing user interest journeys. We provide extensive analysis to understand the effect of different prompting techniques, underlying data, and models. 

\subsection{Experiment setup} 
We evaluate journey naming on  three experimental setups.
\begin{enumerate}
    \item[N1] \textbf{Expert-curated collections}: Data of 100 item collections, named with interesting engaging names from editorial teams. The set comes from the same distribution as (D3) used for prompt-tuning (Section \ref{subsec:data_alignment}), but it is from a different unseen split.
    \item[N2] \textbf{Learning Playlists}: Larger-scale 10,000 playlists, of high episodicity focused in learning-related goals. The set comes from the same distribution as the learning playlists considered for fine-tuning (Section \ref{subsec:data_alignment}); again a different unseen split. As explained before, the names are shorter and noisier, %The names are not chosen from the users with the most care, 
    but still convey meaning about the items saved in the playlists.
    \item[N3] \textbf{Unlabeled Histories}: Larger scale 10,000 unlabeled extracted journeys, from histories of 2,000  users spanning a month (same distribution as E1 in Section \ref{subsec:analysis}). The journeys have been extracted using our ICPC algorithm. These journeys do not have expert or user-associated names. 
\end{enumerate}
%INFERENCE
%feature_lenghts= {inputs: 256, targets: 64} (tokens)
%temperature = 0.0
%beam_size = 1
%max_decoding_steps = 256

%TUNING
%[fine|prompt]_tuning_learning_rate = 3e-5
%[fine|prompt]_tuning_dropout_rate = 0.1
%fine_tuning_steps = 20k
%prompt_tuning_steps = 10k
%prompt_embedding_size = 5 tokens
% It's perhaps worth noting that (N2) is from the same distribution as experiment setup for journey extraction (E2), and (N3) from the same distribution as the (E1) setup. 


For each journey, we concatenate titles of all the items belonging to the journey as input context to the LLMs as shown in Table~\ref{tab:format_examples}, and generate the journey name using different LLMs with different prompting techniques. Unless otherwise specified, we mainly build on top of the LaMDA-137B foundation model \cite{thoppilan2022lamda}. We set the prompt embedding size to 5 tokens. We perform 10,000 prompt tuning steps, and 20,000 fine tuning steps. The learning rate and dropout rate is set to 3e-5 and 0.1 respectively across prompt and fine-tuning. During inference, we set beam size to 1, temperature to 0, max decoding steps to 256 and feature lengths 256 tokens for the input and 64 tokens for the targets.

To quantitatively compare the different naming user journeys approaches, we  rely mainly on BLEURT \cite{sellam2020bleurt} and SacreBLEU \cite{papineni2002bleu} scores.%, and ROUGE \cite{lin2004rouge} score. 
While SacreBLEU measures the  overlap between the generated and the ground truth name, BLEURT, as an embedding-based metric, measures their semantic similarity. For the (N3) setup where we do not have the ground truth names, we propose to rely on a BLEURT score between the concatenated names of input items comprising the user journey and the generated name as the metric.\footnote{BLEU  has been developed and can be interpreted for the domain of machine translation; thus the interpretation of the values for our domain does not have a known reference point. That's why we use it for comparison rather than absolute scores, and we rely on qualitative evaluation as well.}  

\begin{figure}[!th]
    \centering
    % \includegraphics[width=0.45\textwidth]{images/qualitative_journeys.png}
    \includegraphics[width=0.9\textwidth]{images/artphoto.png}
    \includegraphics[width=0.9\textwidth]{images/gokart.png}
    % \includegraphics[width=0.49\textwidth]{images/quality1_new.png}
    \caption{Examples of real extracted and named user journeys through our journey service.
    %\minminc{remove the infinite concept on top of each to reduce clutter. show the four in one column to be more readable.} %\minminc{print the paper out, and see if you can see the texts.}
    %\kc {alalama: consider https://screenshot.googleplex.com/6diNp4VwHDGEonK, https://screenshot.googleplex.com/4MyLHoCwM3JNcxK, https://screenshot.googleplex.com/78wmf7PKbGGQojP, https://screenshot.googleplex.com/5KqR9XHgEdUR6h9}
    }
    \label{fig:example_qualitative}
    \vspace{-0.2in}
\end{figure}


%\kc{Adjust that to (1) only prompting techniques (2) Model architecture, and model size (3) Safety, Interestingness (4) Why journey extraction? (5) Qualitative (6) Recommendation.}
\subsection{Key Result: Prompting LLMs can reason well through user interest journeys.}
As shown in Figure \ref{fig:example_qualitative},
our journey naming service can provide accurate, nuanced names describing the user interest journeys, like \emph{the art of photography}, or \emph{go kart racing}. These qualitative results illustrated are from a prompt-tuned LaMDA-137B model using expert-curated collections as explained in Section~\ref{subsec:data_alignment} (prompt tuning data), used in inference mode on top of real user journeys on an industrial recommendation platform, extracted via our ICPC method.
%aligning LLMs with the user interest journey domain, results in b

%\kc{What should we point to here?} \minminc{maybe show a couple of qualitative results. Figure \ref{}}


%\subsection{Few-shot prompted LLMs can nicely summarize user journeys, and provide related journeys}

%\begin{figure}
%    \centering
    %\includegraphics[scale=0.35]{images/real_journeys.png}
%    \includegraphics[scale=0.13]{images/pizza_construction.png}
%      \includegraphics[scale=0.12]{images/pizza_related.png}
%      \includegraphics[scale=0.12]{images/pizza_description.png}
%    \caption{LLMs have the capabilities of accurately and interestingly naming the user journey, providing related interests / steps of the journey user might want to explore, and provide a detailed description of the journey} 
%    \label{fig:pizza}  
%\end{figure}

%At a glance, Figure \ref{fig:pizza} demonstrates the overall capabilities we have uncovered that LLMs have for naming the user journey, providing related interest journeys when prompted accordingly, and even describing in a detailed fashion what the journey is about. In this paper, we focus our results on the first capability of naming the journey. It's worth mentioning though that for the smaller experimental setup of 100 expertly-named and curated collections, we have compared ground truth description with inferred description, and the BLEU score is \kc{add here the number, or include the figure and reference it}. We can also see that with the prompt, "Other interests worth exploring:" the user can easily delve into other adjacent concepts of this journey, or tangent interest journeys. 

\subsection{RQ1: Which prompting technique performs  best for journey naming?}

\subsubsection*{Prompt tuning on small high quality data outperforms few-shot prompt engineering}

%\begin{figure}
%    \centering
    %\includegraphics[scale=0.35]{images/real_journeys.png}
%    \includegraphics[scale=0.18]{images/bleurt_flanpalm_vs_LaMDA137B_small.png}
%    \caption{Comparison of LaMDA 137B vs FLANPaLMchilla across different input types.} 
%    \label{fig:small_flanpalm_vs_LaMDA}  
%\end{figure}

%\emph{What is the generalization capability when inferring in a more noisy domain?} Given these results in the smaller, higher quality named playlists/journeys, we want to see whether these results would transfer when prompt-tuning/few-shotting from examples of these highly curated names, to the more noisy experimental setups of (B) user-named playlists, and (C) unlabeled user histories. 


\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.33\textwidth]{images/N1_setup_Expert_curated_collections_8.png}
\includegraphics[width=0.33\textwidth]{images/N2setup_Learning_Playlists_4.png}
    \includegraphics[width=0.33\textwidth]{images/N3setup_Unlabeled_Histories_3.png}
    %\includegraphics[width=0.33\textwidth]{images/LaMDA Infiniset_ YouTube Learning Playlists - BLEU.png}
    %\includegraphics[scale=0.15]{images/playlists_ fs_vs_pt_bleu.png}
    %\includegraphics[width=0.33\textwidth]{images/LaMDA Infiniset _ YouTube Learning Playlists _ BLEURT.png}
    %  \includegraphics[scale=0.15]{images/playlists_ fs_vs_pt_rest.png}
     % \includegraphics[scale=0.13]{images/unlabeled_fs_vs_pt.png}
     %\includegraphics[width=0.33\textwidth]{images/LaMDA Infiniset _ Unlabeled Histories _ BLEURT.png}
    \caption{\textbf{Few shot vs. prompt tuning vs. fine-tuning}. (left) Expert collections. (middle) Learning playlists. (right) Unlabeled Histories.}%for prompt-tuned LaMDA 137B vs few-shot LaMDA 137B. (right) Unlabeled extracted journeys. \minminc{remove youtube from the figure title. and use the N1, N2, N3 names as in section 5.1.} \minminc{I think a better organization of the results here might be 3 figures on N1, N2, N3, in each figure we have 6 bar plots, few-shot, prompt tune, fine-tune with BLEU, and BLEURT (in a different color).}} 
    \label{fig:larger_fs_vs_pt}  
\end{figure}
Figure \ref{fig:larger_fs_vs_pt}(middle) and (right) compares the different prompting techniques for LaMDA 137B in the larger experimental setups (N2) and (N3), respectively. We can see that for both setups, prompt-tuning performs significantly better compared to few-shot, as measured both by SacreBLEU and BLEURT scores. In Figure \ref{fig:larger_fs_vs_pt}(left) we also find similar results in the smaller but higher quality evaluation (N1) setup of the 100 expert-curated named collections: prompt-tuning outperforms few-shot prompt engineering both in terms of SacreBLEU and in BLEURT score. 
We also found that few-shot with 5 examples (bleurt 43.28) significantly outperforms zero-shot prompting (bleurt score 31.68). %(\kc{provide percentage}); and (2) prompt-tuning outperforms few-shot prompt engineering both in terms of SacreBLEU and in BLEURT score. %We confirm same results of prompt tuning outperforming few shot when prompting the model of FLAN PaLMChilla as well, as shown in  Figure \ref{fig:effect_prompt_metadata}(right) \minminc{should move the figure up if we want to discuss the result here.}.
%Another observation is that comparing the generalization power of the prompt-tuned LaMDA model in the user learning playlists setup vs the test expertly named curated collections, the SacreBLEU achieved in the latter is significantly higher (~9\%) compared to the one achieved in the more noisy setup (~5\%).




%shows that in the setup of inferring the names of the user playlists, prompt-tuning performs significantly better compared to few-shot which is especially evident as measured by SacreBLEU score.Also, the BLEURT score between inferred journey name and items' titles in the journey is higher in the case of prompt-tuned LaMDA vs few-shot. 


\subsubsection*{Fine-tuning outperforms prompt-tuning in-domain, but prompt-tuning has better generalization capability.}

%\begin{figure}
%    \centering
%    \includegraphics[scale=0.1]{images/ft_vs_pt_2b_unlabeled.png}
%    \caption{Using the same formulation of inference examples, a prompt-tuned LaMDA model outperforms fine-tuned LaMDA. With more dialogue-looking formulation, fine-tuned LaMDA based on user learning playlists outperforms prompt tuning. \kc{Further add figure here  regarding instruction tuning.}}
%    \label{fig:pt_vs_ft_LaMDA}
%\end{figure}

Fine-tuning is the default strategy for aligning LLMs to new domains. We tested whether fine-tuning LaMDA 137B on 20,000 user-generated playlists (with input the items and output the corresponding user-given names) could outperform learning the prompt embedding based on the  (D3) smaller dataset of expertly curated named collections. The answer is: it depends. Based on results in Figure \ref{fig:larger_fs_vs_pt}, we find that fine-tuning outperforms prompt tuning for the (N2) evaluation setup where examples come from the same distribution as fine-tuning examples, aka Learning Playlists data. However, testing the generalization power of both prompting techniques in (N3) setup of unlabeled histories, prompt tuning outperforms fine-tuning. Also, from setup (N1) we find that  prompt-tuning with small in-domain examples outperforms fine-tuning with out-of-domain large scale data.

%\kc{Add more here.} %With an identical formulation of passing examples in inference mode to the LLM, prompt tuned LaMDA outperforms fine-tuned LaMDA. However, when we formulate the examples more in the form of a multi-turn conversation, or even better a dialogue of questions and responses, the fine-tuned LaMDA model outperforms the prompt-tuned one. This is not too surprising, as the pre-trained LaMDA models has a lot of data in the form of dialogue, thus potentially making the model more capable to reply when prompted in a  conversational format. \kc{Here we will update with the equivalent models. } 


%\subsubsection{Instruction tuning significantly improves LLMs performance.}
%\kc{Not sure if that's a valid highlight we have seen from our results.}

\subsection{RQ2: Which underlying model is better, and under which circumstances?}

\subsubsection*{Effect of model size}
\begin{figure}
    \centering
    \includegraphics[width=0.33\textwidth]{images/Effect_of_model_size_2.png}
    \includegraphics[width=0.33\textwidth]{images/comp_prompt_tuned_1.png}
    \includegraphics[width=0.33\textwidth]{images/Comparison_of_Few_shot_prompted_model_architectures_2.png}
    %\includegraphics[width=0.33\textwidth]{images/model_size_BLEU.png}
    %\includegraphics[width=0.33\textwidth]{images/model_size_ BLEURT.png}
    %\includegraphics[width=0.33\textwidth]{images/LaMDA _ Unlabeled Histories _ BLEURT.png}
    
    \caption{(left) \textbf{Effect of model size.} (middle, right) \textbf{Effect of model architectures.}}
    \label{fig:effect_model_size}
\vspace{-0.1in}
\end{figure}

Figure \ref{fig:effect_model_size}(left) compares how prompt tuning different sized LaMDA models affects the quality of generated journey names, considering the large-scale setups (N2) and (N3). One surprising observation is that while the performance on (N2) learning playlists suggests prompt tuning larger sized model leads to better naming quality, there is not a monotonic improvement on the (N3) unlabeled histories case. % of the metrics achieved by the prompt tuned model with increase in model parameter size. %Another observation is that for different evaluation metrics (e.g., SacreBLEU vs BLEURT) the order of best-performing models changes; e.g., a prompt-tuned LaMDA 137B model outperforms other sized-variants in terms of BLEURT, but has the lowest SacreBLEU score. 
Overall, we explain these results by hypothesizing that when increasing the model size, on the one hand, the model has more capacity to infer good quality labels; on the other hand, the conditioning of model on the learned prompt embedding might become less prominent. Another hypothesis is the difference in the data among the two setups: (N3) compares output to input, while (N2) compares output to human labels. This trade-off among model size and prompt tuning needs further research investigation.

\subsubsection*{Effect of different model architectures}
%\kc{if needed update results, and include gpt3 as well.} 
In Figure \ref{fig:effect_model_size}(middle), we compare prompt-tuned models: PaLMChilla 62B, and its corresponding instruction tuned variant Flan-PaLMChilla 62B, with LaMDA 137B. We see that for both (N2) and (N3) setups, LaMDA 137B achieves the best BLEURT score. We also see that the performance of instruction-tuned PaLMchilla does not differ much from its non-instruction-tuned counterpart. 
Interestingly, when comparing few-shot prompted models FLAN PaLMChilla 62B with LaMDA 137B (Figure \ref{fig:effect_model_size}(right)), the order is reversed: FLAN PaLMChilla  outperforms LaMDA in (N2). We think that the instruction tuning of the former makes it better in following the few-shot prompting. Either way, both few-shot prompted models achieve lower BLEURT compared to the worst prompt-tuned model in the (N2) setup shown in Figure \ref{fig:effect_model_size} (middle).
%In Figure \ref{fig:effect_model_size}(right), we compare few-shot prompted models: FLAN PaLMChilla 62B with LaMDA 137B  in the (N2) learning playlist setup. We see that FLAN PaLMChilla achieves higher BLEURT. \minminc{explain why.}

%\begin{figure}
%    \centering
    %\includegraphics[width=0.33\textwidth]{images/Model Architecture _ YouTube Learning Playlists _ BLEURT.png}
    %\includegraphics[width=0.33\textwidth]{images/Few-shot prompted Model Comparison. .png}
    %\includegraphics[width=0.33\textwidth]{images/Prompt-Tuned Model Comparison. Learning Playlists.png}
    %\includegraphics[width=0.33\textwidth]{images/Prompt-tuned Model Comparison. Unlabeled Histories.png}
    %\caption{\textbf{Model architecture comparison.} (left) Comparing few-shot prompted; and (middle, right) prompt-tuned models. \minminc{The bleu and bleurt mix in the left figure can be confusing. how about stick with bleurt?}}
    %\label{fig:model_arch}
%\end{figure}

\subsection*{RQ3: How construction of the prompt affects the quality of generated interest names?}

\subsubsection*{Which metadata are useful to be part of prompt?} Figure \ref{fig:effect_prompt_metadata} shows for (N1) setup, how different ways of representing the items: (1) using item titles/names, or (2) using keywords representing the playlist, or (3) with both item names and playlist keywords (as discussed in Table \ref{tab:format_examples} for structured prompts) interact with different prompting techniques. Overall, we find that the titles of the items is the most informative feature, with some additive value provided when including playlist keywords. %This is why in most experiments, u
Therefore, unless specified otherwise, we infer journey name given only titles metadata.

%\begin{figure}
%    \centering
    %\includegraphics[scale=0.35]{images/real_journeys.png}
    %\includegraphics[width=0.33\textwidth]{images/Effect of prompt metadata.png}
    %\includegraphics[width=0.33\textwidth]{images/Effect of prompt tuning datasets.png}
    %\includegraphics[width=0.33\textwidth]{images/bleu_LaMDA137B_small.png}
    %  \includegraphics[width=0.33\textwidth]{images/bleurt_LaMDA137B_small.png}
    %  \includegraphics[width=0.33\textwidth]{images/bleu_flanpalm_small.png}
      %\includegraphics[scale=0.1]{images/bleurt_flanpalm_small.png}
    %\caption{(left) \textbf{Effect of different prompt metadata} in (N1) setup.  (right) \textbf{Effect of  prompt-tuning datasets} in (N2) and (N3) setups. 
    %} 
    %\label{fig:effect_prompt_metadata}  
%\end{figure}

%\begin{figure}
%    \centering
    %\includegraphics[scale=0.35]{images/real_journeys.png}
    %\includegraphics[scale=0.1]{images/bleu_flanpalm_small.png}
    %  \includegraphics[scale=0.1]{images/bleurt_flanpalm_small.png}
    %\caption{(left) BLEU (right) BLEURT for FLANPaLMchilla across different input types.} 
    %\label{fig:small_flanpalm}
%\end{figure}

\begin{figure}
    \centering
    \begin{minipage}{0.33\linewidth}
    \includegraphics[width=\textwidth]{images/Effect_of_prompt_metadata.png}
    \caption{Effect of  prompt metadata.}
    \label{fig:effect_prompt_metadata}  
    \end{minipage}
    \begin{minipage}{0.33\linewidth}
    \includegraphics[width=\textwidth]{images/Effect_of_prompt_tuning_datasets.png}
    \caption{Effect of prompt-tuning datasets.}
    \label{fig:effect_prompt_tuning_data}  
    \end{minipage}
 \begin{minipage}{0.33\linewidth}
    %\includegraphics[width=0.5\textwidth]{images/Using only last five items vs all items to infer journey name.png}
    %\includegraphics[width=0.5\textwidth]{images/Using only last eleven items vs all items to infer journey name.png}
    \includegraphics[width=\textwidth]{images/Effect_of_number_of_items.png}
    \caption{Effect of number of journey items. %\minminc{can we use bleurt score here?}
    }
    \label{fig:journey_length}
    \end{minipage}
    %\includegraphics[width=0.33\textwidth]{images/safety_etc_twosetups.png}
    %\includegraphics[width=0.33\textwidth]{images/safety_etc_models_sall.png}
    \vspace{-0.1in}
\end{figure}
\subsubsection*{Effect of prompt tuning data on success of learned prompt embeddings.}

%\begin{figure}
%    \centering
%    \includegraphics[width=0.33\textwidth]{images/diff_prompt_data_playlists_rest.png}
    %\includegraphics[width=0.33\textwidth]{images/diff_prompt_data_unlabeled.png}
    %\includegraphics[width=0.33\textwidth]{images/diff_prompt_data_playlists_bleu.png}
%\caption{Effect of prompt tuning data. (left, middle): Learning Playlists setup.  (right) Unlabeled Histories setup. \minminc{let's stick with bleurt.} }
%    \label{fig:diff_prompts}
%\end{figure}
As expected, the quality of the data used to learn the prompt embedding plays a key role in how successful prompt tuning LLMs can be. In Figure \ref{fig:effect_prompt_tuning_data}, we compare how learning the prompt on top of three different small quality datasets generalizes in the task of inferring journey names for the larger (N2) and (N3) experimental tasks. The prompt tuning data are the (D1) user interviews, (D2) user collections, and (D3) expert-curated collections, as described in Section \ref{subsec:alignllms}. 
In both (N2) and (N3) setups, we see a big difference in performance based on the data we use to learn the prompt, with prompt embeddings learned from expertly curated names of collections providing the highest generalization capability. We argue that this is the case because the expertly named collections provides higher quality data to learn the prompt compared to user provided names, which tend to be more noisy, especially in the context of an interview where recipients might provide data of mixed quality. These results also point to the potential of mixed methods, i.e., mixing expert-provided labels, with a subset of higher quality user-provided labels, for enabling LLMs to accurately describe user interests.  

\subsubsection*{Effect of journey length.} We also conduct experiments to understand the number of items in the journey that should be included in order to generate a good name. Figure \ref{fig:journey_length} shows that if we generate names only given the last five items in the journey, the SacreBLEU score between ground truth and generated name is significantly lower compared to if we were to use all the items in the journey\footnote{This comparison is done limiting to journeys that have more than five items, in the (N2) setup.}. However, when comparing journey names as inferred by the last eleven items only (now in histories of more than eleven items), there is little drop in performance compared to using all items in journeys. This can be a guiding point to reduce the context length in generating journey names. % cost of number of items to keep track of to generate the name.  


%\subsubsection*{What if we include instructional data?} \kc{again, here or above?}

\subsection{RQ4: How safe and interesting generated user journey names are?}

As pioneered in \cite{thoppilan2022lamda}, besides the accuracy of responses generated by LLMs, other evaluation dimensions should be considered as well. These include how safe/responsible the responses are; how interesting they are; whether they are sensible; and whether they are specific enough, with many of these dimensions competing one against the another (e.g., the safer the response, the less interesting it might be). %Given this background, 
We utilize the already trained LaMDA scorer \cite{thoppilan2022lamda} (without the prompting done to align to the journey interest domain), as the imputation model for the aforementioned dimensions. . % each of these scores, which represent probability of being safe, interesting, sensible, and specific. 
Figure \ref{fig:safety} plots the imputed scores for the generated, by the prompt-tuned LaMDA-137B model, names, in the three setups (N1), (N2) and (N3). Our key takeaway is that the degree to which the generated journey names are safe/ interesting/ and so on, is largely affected by the underlying input given in inference to produce the names. This is evident by the fact that the more in-the-wild unlabeled histories have names which have lower safety score compared to names produced by the same model for the user-curated playlists, or the expert-collections. %We also see that in the case where experts are curating and naming collections, the inferred by LLMs names are near perfect safe, very interesting and specific, with lower sensibility scores, which might be as these names are meant to draw attention rather than completely factually describing the items in the collection.     



%\subsubsection{Qualitative Examples}%: Prompted models can nicely summarize real user journeys.}
%\kc{Add table, and potentially add what the description is.}
%\subsection{Towards demonstrating the value of extracting & naming journeys for improved recommendation experience}

%\subsection{Visualization of journeys}

\subsection{RQ5: Do we need  journey extraction, or can we rely on LLMs on both journey extraction \& naming?}
%\kc{Add results here comparing for each YouTube history what's the corresponding.}

%\begin{figure}[!t]
%    \centering
%    \includegraphics[width=0.4\textwidth]{images/value_of_extraction.png}
%    \caption{Value of first extracting journeys, before naming them via LLMs.}
%    \label{fig:extraction_value}
%\end{figure}
  
A natural question that might arise to the readers is that given LLMs evidently can be used to generate nuanced interesting names of the interest journeys users are pursuing, why not also task them with the job of both extracting and naming simultaneously? To answer this question, we use the evaluation setup (N3). %where we have the interaction histories with items over a month of 2,000 users. When running our journey extraction module on top of the raw histories, as described above results in ~10K journeys.
The approaches we compare are: (1) Providing the whole user history to the LLM and asking the model to name the interest journeys the user is pursuing. (2) Extracting journeys using our ICPC, and concatenating the journey groups (compared to the mixed history in (1)) at once in a single inference to the LLM and asking it to name the journey groups. (3) Naming each extracted group separately, with a different LLM call per journey. We compute the BLEURT score between the whole input history and the concatenated journey names as the final evaluation score and compare the three approaches. It's evident from Figure \ref{fig:extraction_value} that the LLM can generate significantly better journey names when it's only given the journey-specific history, thus further validating the need for our journey extraction component in the journey service.

\begin{figure*}%{\textwidth}
    \begin{minipage}{0.33\linewidth}
    \includegraphics[width=\textwidth]{images/Imputation_metrics_on_generated_names.png}
    \caption{Imputed aspects for names. %\minminc{add label for y axis}
    }
    \label{fig:safety}
    \end{minipage}
  \begin{minipage}{0.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/value_of_extraction.png}
    \captionof{figure}{Value of extracting journeys, separate than naming.}
    \label{fig:extraction_value}
  \end{minipage}
  \begin{minipage}{0.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/Journey_aware_recommendations_headroom_2.png}
    \captionof{figure}{Headroom of journey-aware recommendations.}
    \label{fig:recommendations_headroom}
  \end{minipage}
  \vspace{-0.1in}
\end{figure*}
\subsection{RQ6: Can the extracted and named journeys enable an improved recommendation experience?}
Lastly, we provide some early analysis on the degree to which a user's journeys can be better assisted when the recommender is aware of the underlying journeys. We compare the  journeys extracted from real user histories over the period of a month (same setup as N3) with the recommendations given to the user the day after the month on the industrial platform. For each journey of a user, we compute the similarity of the average salient terms embedding of the journey and that of all the recommended items\footnote{For computation purposes, we reduce comparison of each journey with each recommended item, to comparing with the entire recommendation set}. %We can then compute for each user the average similarity between the infinite concepts embedding of the journey history items and all provided nominations. 
When the similarity is larger than a threshold (set to 0.2), we track the journey as being served. We can then compare this with a new recommendation process using our journey service and search: 1) we extract journeys from the one-month user history and name the extracted journeys using prompt-tuned LaMDA 137B on (D3); 2) we generate recommendations for each journey through searching the platform using the generated journey name. %\minminc{need to say something about the total recommendation items are kept similar between this new setup and the production}. 
We then compute the similarities between these new journey-aware recommendations and journeys for comparison.  %the case when for each journey we map the journey name as outputted by prompt-tuned LaMDA to recommendations via calling Search.
We can see in Figure \ref{fig:recommendations_headroom} that on average over a hundred sampled users, 
%\minminc{with total X journeys}
around 1 out of 10 journeys is served (0.102) under the current recommendation system. This number is significantly improved when the recommender is journey-aware (0.253). We also report the average similarity score between journeys and candidates (without the thresholding). We can see that overall, the provided recommedation candidates have higher  similarity in the case of journey aware nominations (0.127 vs 0.099). Of course, to fully answer this question, ideally we need novel recommendation approaches mapping the journeys to recommendations. We also need A/B user facing experiments to measure the value added to the user. Both will be part of our future work. Nevertheless, these early results already point to headroom of improving recommendations via making them aware of user interest journeys.

%\kc{The value of naming via LLMs via other approaches:Can we compare with legos? Can we compare with salient terms representing the journey? }

%\kc{Also add here the side-by-side evaluation.}

%\kc{Other: Prompted models can also generate longer descriptions around user journeys.}
%\kc{Add here the playlists results too.}



==> Paper_ Extracting and Naming User Journeys for Companion Recommenders (3)/uxr.tex <==
%A recommendation system that aims to assist users throughout their lifelong journey should reflect what real people are pursuing in their life, and how they want to be assisted. Therefore, 
To build recommender systems that are able to assist users on their journeys, we started by launching a series of user research studies consisting of online surveys and user interviews to understand the types of journeys users pursue. %Study protocols underwent internal research review and attained approvals before being administered with participants. 
Informed consent from study participants was collected in accordance with company user data and privacy policies, which adhere to ethical research standards on human participants policies. Furthermore, all user data was de-identified by replacing names with randomized numbers and securely stored. 

 
% \begin{wrapfigure}{l}{0.32\textwidth}
%     %\centering
%     %\includegraphics[scale=0.35]{images/real_journeys.png}
%     \includegraphics[width=0.3\textwidth]{images/real_journeys_youtube.png}
%     \caption{(Sample real journeys described by users. }%\kc{add this in sorted popularity.}
%     \label{fig:real_journeys}

% \end{wrapfigure}

% \begin{figure}[!t]
%     %\centering
%     %\includegraphics[scale=0.35]{images/real_journeys.png}
%     \includegraphics[width=0.3\textwidth]{images/real_journeys_youtube.png}\hspace{10pt}
%       \includegraphics[width=0.3\textwidth]{images/taxonomy_interests.png}
%     \caption{(left) Sample real journeys (right) Taxonomy of valued journeys uncovered by clustering text user responses via UMAP \cite{mcinnes2020umap}.%\kc{add this in sorted popularity.}
%     } 
%     \label{fig:real_journeys}
%       \label{fig:valued_journeys}

% \end{figure}
%\subsection{Goals \& User Research Study Setup}
%\noindent \textbf{Goals.} 
% Our goals are two-fold. First, to gain insight into our target domain, namely the space of journeys users are pursuing, how they describe them, the type of assistance they need. Two, to identify ways to construct our experiments and evaluate our experimental results, namely how many journeys users are pursuing, in which frequency, and at what granularity and way they specify/describe them. 

%We launched a series of user research studies consisting of online surveys, and user interviews to understand the types of journeys users pursue. We use terms "interest journey" and "journey" interchangeably in this section.%, as this is what was shown on the surveys. %support and decide on the types of journeys we want to assist. 
\noindent \textbf{Setup.} 
We sent %four 
online surveys to approximately $12,000$ users of an online platform, (a representative sample of the US internet user population aged 18-65+), with the goal of answering the questions: (Q1) If and how people use existing online platforms to pursue their journeys 
%\minminc{how was journey described in the survey to users? -> alalama: added below}?
(Q2) What types of journeys people pursue online? 
Based on the analyzed survey data, we set up in-person interviews with a small cohort (N=9) of survey respondents who had multiple journeys to better understand: (Q3) What are the highlights and pain points of pursuing journeys on the internet? and (Q4) How do their journeys evolve? %\minminc{"in a personalized way" seems to revealing the answer already} \kc{double-check if the platform here is only one or not}.
In the surveys, we framed journeys in terms of real-life interests or goals that the online platform has helped users pursue in a meaningful way. 

%To achieve our goals of better assisting people's journeys via recommenders, we first need to understand: ,  
%Based on the analyzed survey data, we % adapted user interview questions for question three and four, and  
%interviewed a cohort of survey respondents \kc{how many?} with multiple journeys. 

%\subsection{Research Insights}
% \begin{wrapfigure}{l}{0.32\textwidth}
% %     %\centering
% %     %\includegraphics[scale=0.35]{images/real_journeys.png}
% %     \includegraphics[width=0.3\textwidth]{images/real_journeys_youtube.png}\hspace{10pt}
%       \includegraphics[width=0.3\textwidth]{images/taxonomy_interests.png}
%     \caption{Taxonomy of valued journeys uncovered by clustering text user responses via UMAP \cite{mcinnes2020umap}.%\kc{add this in sorted popularity.}
%      }
%       \label{fig:valued_journeys}
%  \end{wrapfigure}
\begin{figure}%{l}{0.62\textwidth}
%     %\centering
%     %\includegraphics[scale=0.35]{images/real_journeys.png}
%     \includegraphics[width=0.3\textwidth]{images/real_journeys_youtube.png}\hspace{10pt}%
        \includegraphics[width=0.3\textwidth]{images/real_journeys_youtube.png}
       \includegraphics[width=0.3\textwidth]{images/taxonomy_interests.png}
    \caption{(left) Sample real journeys described by respondents. (right) Taxonomy of valued journeys uncovered by clustering text user responses via UMAP \cite{mcinnes2020umap}.%\kc{add this in sorted popularity.}
     }
      \label{fig:valued_journeys}
 \end{figure}
 
\noindent \textbf{Insight 1: \textbf{People value content related to entertainment, learning, and community engagement.}}
%We asked over two thousand respondents \kc{what happened to the 12,000 above?} to describe their valued journeys on the platform and got 1612 valid responses. The results were mapped onto a two-dimensional space using UMAP (Uniform Manifold Approximation and Projection for Dimension Reduction) method \kc{Add reference}, the resulting visualization can be divided into roughly nine categories as shown in Figure \ref{fig:valued_journeys}. %including:% \kc{Include visualization in Appendix, or here}: 
%\begin{itemize}
%    \item DIY projects (i.e., sewing, knitting, %woodworking, interior renovation);
%    \item Learning new skills (i.e., language, coding, certificates, music production, game design);
%    \item Entertainment/hobbies (i.e., gaming, photography, music, film);
%    \item Well-being (i.e., mental health, relationships, healing, self-improvement);
%    \item Travel (i.e., trip planning, travel inspirations, camping, guides);
%    \item Maintenance/repair (i.e., home maintenance, car repair, hardware repair);
%    \item Fitness (exercise, yoga, meditation);
%    \item Parenting/care (taking care of children, pets, and plants);
%    \item Cooking (recipes).
%\end{itemize}
%We found a lot of concentrated results in the learning and entertainment categories.%, and further confirmed this in a separate survey. % -- two categories with existing labels \kc{Connect this with our main text of which journeys we choose to cluster, and mention about these scores} we can utilize in our recommendation pipeline. 
%\kc{which survey are we referring to here? Is it the LTV or one we run? -- all the surveys we refer to here are from the 4 separate surveys we ran, corresponding to the 4 sections at: go/subJourneySurvey}, 
Figure \ref{fig:valued_journeys} (left) shows example real journeys as described by our respondents. Figure \ref{fig:valued_journeys}(right) shows the resulting taxonomy of valued interest journeys i.e., journeys they pursue and find satisfactory, by clustering the provided responses via UMAP \cite{mcinnes2020umap}, and identifying  roughly nine emerging themes. In a separate survey, we confirmed that entertainment (50 percent) and learning new skills (34 percent) are among the top valued journeys, 
%Entertainment accounts for $50\%$ of valued journeys, learning new skills $34\%$, % are among the top content types users find valuable on the platform. 
and other dimensions include physical and mental well-being, caring for others, and community building etc. 
% This uncovered taxonomy confirms that users do indeed pursue real-life journeys on recommender platforms, and the provided dimensions can provide useful insights for deeper user understanding. 
%In one survey, 
%Respondents listed "engaging in a community" among the top reasons they value certain types of content. 
%When exploring a niche interest, people often engage with a community of subscribers, content uploaders, and commentators on the platform, which often leads to offline relationships.
%Together, these insights lead us to focus our experiments on extracting journeys  from interactions with high predicted long-term satisfaction scores. This satisfaction score is imputed by models trained on user surveys measuring the degree to which items provide the user with lasting entertainment, learning new skills, and social belonging.

\noindent \textbf{Insight 2: \textbf{People pursue multiple interest journeys concurrently  %\footnote{We use terms interest and interest journey, in the notion described in Section \ref{sec:formulation}, aka. a stickly valued interest, and its evolution in a personalized way respectively.}  
over long periods of time.}} 
Our surveys confirm that users do pursue real-life journeys on recommendation platforms. 
About $66\%$ of survey respondents used the platform recently to pursue a journey they valued. %, confirming that recommenders are used to assist real-life journeys. 
Out of the $66\%$, about 8 in 10 consumed content relevant to a journey for more than a month, with half saying some journey lasts for more than a year. 
%The same survey respondents also reported high consistency in their content consumption behavior. 
% In terms of consumption frequency, %Over half of them reported consuming contents with high consistency over the time span they chose, another 30 percent reported some consistency. This insight provided us with a good time frame reference to define a valuable long-term interest journey, with our initial experiments looking at user histories of a month or more. 
People reported exploring multiple journeys simultaneously, with 7 in 10 pursuing one to three journeys and 3 in 10 exploring 4 or more in a single session. The large majority reported both exploring new valued interests and continuing existing ones. %of people need assistance both in exploring new and pursuing existing valued interests simultaneously.
%65 percent of these respondents reported exploring new and existing valued interests simultaneously.  This insight suggests the need to both support existing journey continuation and exploration of new journeys.%; and that journey extraction from their existing interactions can be helpful to organize content by journeys.




\noindent \textbf{Insight 3: \textbf{People rely more on explicit actions to find content relevant to their interest journeys.}} %\kc{Perhaps completely remove, or rephrase so that it matches the text.} We see a trend of short-form video platforms taking off among internet users. These platforms often prioritize exploratory content over explicit user actions. For instance, a few platforms reduced subscription and search features in favor of autoplay and infinite playback feeds, % \kc{We need to define this or bottomless feeds}, increasing engagement and watch time. However, 
Half of our survey respondents picked the search bar as the most-used feature to pursue their journeys, compared to $20\%$ who relied on the recommendation feed, indicating inefficiency in existing recommenders in assisting user interest journeys, and the opportunity for providing more user control in recommendation experiences \cite{jannach2017user}. % This motivates us to build journey-aware recommendation experience which allows users to interpret and control recommendations to better pursue their interest journeys. % interpretable, controllable, and human-like % This indicates the opportunity for more user control in the recommendation experience, further motivating our thesis to make recommenders aware of users interest journeys, expressed in an interpretable, human-like way.

%Though 22 percent of platform users reported liking most of the recommendations on their home feed, and 53 percent say they like some recommendations--- 1 in 4 users say they rarely, or never click on their home feed content. This presents us with an opportunity to provide more explicit control on people's home feeds related to their extracted long-term user interest journeys, empowering them to take explicit actions relevant to their journeys, which can in turn  improve the recommender results.%\kc{Took out the language modeling part.}%With our large language models, we have an opportunity to give people natural language understandings for their recommendations, empowering them to take explicit actions in improving the recommender results. 

\noindent \textbf{Insight 4: \textbf{People's journeys are nuanced and evolve in a personalized way.}}
Our in-person interviews uncovered a lot of nuance in % the complexity and fluidity of 
people's journeys. For example, one participant placed their interest journey in the general category of "gardening". As they dived deeper, they described it in much more nuanced phrases, i.e., "designing hydroponic systems for small spaces."  Another aspect uncovered was the right specificity people identify with, e.g.,   "greenhouse designs for cold climates" was deemed irrelevant for someone pursuing indoor gardening. %\minminc{nuance and specificity here seem to be talking about the same thing.} 
Finally, participants mentioned how their interest can change based on offline and on-platform interactions. In other words, there are not two identical journeys between users, calling for personalized treatments. % Journey is a personalized notion. % thus making personalisation preferred over a canonical journeys approach.  
%With our natural language processing capabilities, 


%There's an opportunity to pinpoint niche journey descriptions to assist people's journeys as they evolve. However, there's a higher risk of This underlines the importance to extract journeys at the right granularity, and to use natural language to describe niche journeys as they're evolving. 


Together these research insights guide our methods and experimental setup, and provide motivation towards a recommendation experience that can offer  interpretability and control, enabling users to  pursue their interest journeys.


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> metrics_methods.tex <==
 \subsection{Desiderata}
\label{subsec:desired_properties}
\kc{Consider moving to metrics section}
%Reiterating from Section \ref{sec:formulation}, we want to assist long-term journeys that involve multi-step explorations of interest/topics people want to spend more time on. % and expect to engage with for more than a month. 
%For this, we argue the need for a service mapping for each user their overall history (lifelong journey) into possible journeys. %(Figure \ref{fig:journey_pictorial}). 


%from the user history sequences of items that should be all about the same interest journey. 
%come up with a splitting of the lifelong history of the user to sequences, where each sequence covers the above properties. 
%We first specify our design goals, which will largely guide the desired properties for the extracted journey clusters. %When designing a service  mapping each user's  overall history into possible journeys, the goals we have for the expected improvements will largely guide the design. 
The goals of journey extraction are two-fold:
\begin{enumerate}
    \item[(D1)] Enable better recommendation quality and user experience
    \item[(D2)] Enable better organization of content by journeys
\end{enumerate}
%\subsection{Desiderata for journey entity extraction}
\label{sec:desiderata}
We specify the desired properties for the extracted journeys:
%To reflect the above design goals, . %This way we can inform whether existing metadata grouping content are a good fit for journeys, and prescribe the preferred approach to extract journeys.  
% and its applications. 
%\begin{figure}
%  \includegraphics[width=0.5\textwidth]{images/sequence.png}
%  \includegraphics[width=0.5\textwidth]{images/sequence2.png}
%  \caption{Identify that the user is on two journeys: the blue and the red one. A crucial decision is based on which metadata / representation we should decide what is red and what is blue? Because if we look at too high of a level (less granular) red and blue might be merged into one single sub-journey. And if we look too low of a level more granular, we might end up with multiple shades of blue and multiple shades of red, whereas in reality it's just two journeys we need to support well: blue and red.  }
%  \label{fig:journey_pictorial}
%\end{figure}
%\begin{itemize}

    \noindent \textbf{Thematic coherence/ High Precision:} Each extracted journey should only contain items about the same thematic need; %it shouldn't contain items from other journeys. 
    \begin{equation}
        \text{Precision} = \frac{\text{\# of well retrieved journey items in the cluster}}{\text{\# items in the extracted cluster}}
    \end{equation}%which preserve the thematic coherence of the journey; it shouldn't contain items from other journeys
    %When a journey is about another semantic meaning it should be pulled apart into another journey. E.g., "learning the ukulele" is a different journey from "learning the guitar".
    \noindent \textbf{High Recall:} Each extracted journey should ideally retrieve all related items from the user history which are a part of the same journey. %Can be viewed as high coverage, i.e., covering all items/concepts which should be a part of the journey.
    \begin{equation}
        \text{Recall} = \frac{\text{\# of well retrieved journey items in the cluster}}{\text{\# items in the ground-truth journey}}
    \end{equation}
    \noindent \textbf{Right granularity:} %The extracted journeys should be neither too general (e.g., "learn music"), nor too specific (e.g, "learn A, B, C chords on ukulele"), but rather at the right granularity (e.g., “learn the ukulele”), to be useful. 
    The extracted journeys should neither be too general, nor too specific to be useful for changing the recommendations accordingly. Finding the right  granularity is challenging, it however does manifest in the precision and recall tradeoff---when too coarse, many journeys will be unnecessarily merged, thus increasing recall while deteriorating precision; When too fine-grained, precision will be increased (at its limit each interaction is a separate journey), but recall will suffer. 
    %Measuring granularity is hard; thus, it can be indirectly measured via having both high coherence and high recall.
    
    Other metrics that can be used as proxies for granularity evaluation are %\textbf{cardinality-related metrics}, including 
    \begin{itemize}
        \item \textbf{\# of journey clusters per user}: based on our user research, most users pursue 1-3 interest journeys; thus more clusters per user could point to too fine-grained clusters; 
        \item \textbf{\# items per journey cluster}: clusters with too few items can hardly justify as long-term journey, as this should span multiple interactions.
    \end{itemize} 
    By definition we will be eliminating clusters with only one-item, thus other proxy  metrics are:
    \begin{itemize}
        \item \textbf{\# unclustered items per user}, and
        \item \textbf{\# users without journey clusters}.
    \end{itemize}
%    Especially the \# of journey clusters per user can reveal whether too many journeys are extracted, as from our user research we know that the majority of users at a point in time pursue 1-3 interest journeys. Also, a cluster with just a couple of items can hardly justify as long-term interest journey, spanning multiple interactions.
%\begin{equation}
%\textbf{Cardinality} = \text{Total \# of Extracted Journeys per user}
%\end{equation}, 
%\begin{equation}
%\textbf{Per-journey Cluster Cardinality} = \text{\# of Clusters per journey}
%\end{equation}, 
%\begin{equation}
%    \textbf{Documents }
%\end{equation}
%    as well as not too many journeys
    % Granularity affects precision and recall/coherence. When too coarse, many journeys will be merged into one by the method, thus increasing recall but resulting in poor precision. When too fine-grained, precision will be perfect (at it's limit each item is a separate journey), but recall will suffer. It also affects cardinality, as too granular clusters will lead to more journeys. Minimizing cardinality though is not an objective on its own, as this will 
% Measuring granularity is hard; thus, it can be indirectly measured via having both high coherence and high recall, as well as not too many journeys. Another way to indirectly measure it is via the number of items belonging to a cluster, as too many clusters consisting of too few items would probably mean poor granularity, and . Mean # clusters per journey. 
%    I.e., we want the journeys to be at the granularity of “learn the ukulele”; not “learn A, B, C chords on ukulele”, but also not “learn a musical instrument”. Too granular of journeys might end up containing only a handful of items, and too broad of journeys might merge too many unrelated journeys together. Either fallback would minimise the benefits of journey extraction.
%    \item \textbf{High Precision}: Each of the journeys should contain only items which preserve the thematic coherence of the journey; it shouldn't contain items from other journeys.
    \noindent \textbf{Intra-Journey connectivity} and \textbf{Item/Metadata <> Journey connectivity}: The extracted journeys should reflect the \emph{structure} among items belonging to them, and the structure among journeys.
%    Related  journeys should live close together in the semantic/embedding space, so that related journeys can be explored \cite{}.
%    \noindent \textbf{Comparability of journeys <> items / content metadata:} Ability to represent journeys in the same space as items, and as other metadata, to allow user exploration across different entity types.

    \noindent \textbf{Interpretability:} Each journey should have an associated label, or set of concepts describing what the journey is about. %This will facilitate the content organization by journeys design goal.
%    \item \textbf{Low Cardinality:} Related to the right granularity property, at every point every user is typically on journeys in the order of tens, not more. This is also crucial to control the complexity introduced when including journeys  to adapt recommendations.
%\end{itemize}

% Structure between content items, and among journeys, as in being able to compare , and visualizing the key concepts each journey is about.  
% 

%https://docs.google.com/document/d/118klhbcOr1Kz2EekJjrRyiubr1z7xVAUXkyQ1-AOG_k/edit?resourcekey=0-ktyTB8oqKuNB4Fe2ktLZJQ#heading=h.b1ku1ghop8on

\subsubsection*{How desiderata satisfy the design goals:} We argue that the properties of thematic coherence, high recall, and right granularity are very important for both design goals. Imagine a journey extracted at too fine granularity of "A, B, C chords"; or of low coherence containing irrelevant items into a high-valued journey; or of low recall not realizing that user interactions span the same journey. This could hardly result in an improved user experience, or good content organization. Furthermore, the ability to express items, content metadata, and journeys in the same space, can enable the recommender to find items tailored to the journey, and allow user explore related journeys as well---both crucial for a good recommendation experience (D1). The ability to interpret what the journey is about in human readable format can allow the system explain to users content recommendation through the lens of interest journeys, and if right, have the users feel understood (D2). %that the system gets what their interest journeys are.  will feel that the system understands what their real-life goals are, and the bigger interest arcs they are pursuing

%E.g., imagine a journey being extracted at the level of <A, B, C> chords. 

%\subsubsection{Enable better recommendation quality and user experience} 
%Our main goal is to improve the recommendation quality, and the user experience. The hypothesis is that conditioning the recommendations on the journey that the user is on will both allow the model to better figure out the recommendations they can give, and in the process give the user more journey-aware recommendations. The ability to express both items and journeys in the same space can allow for finding items which are a good match. Also, the ability to explore related journeys, and express in the same space other content entities (such as creators, genres, and so on) can enable better user exploration allowing users to traverse the content space much more effectively. Furthermore, being able to extract the journeys at the right granularity is important, where each extracted journey is all about the same longer-term interest, and it's neither too broad nor too specific. 

%\subsubsection{Enable better organization of content by journeys}
%We want to better organize the abundance of potential content to recommend to user by their journeys. This way, the users 
%\begin{enumerate}
%    \item will feel that the system understands what their real-life goals are, and the bigger interest arcs they are pursuing;
%    \item will find easier what they are looking for related to their interests, and be able to better control their  experience. 
%\end{enumerate}
%This is related to explaining to users why they see certain content through the lens of long-term user journeys, and giving them control as to whether they continue pursue certain long-term interests or not. 
%Thus, being able to explain to users why they see certain content through the lens of long-term user journeys, as expressed in natural language, is important.
%being able to explain journeys through concepts in natural language space is important. %Note that this goal can be seen as rather a means to achieve even more effectively the first goal of improved user experience. 

